Robust and On-the-fly Dataset Denoising for Image Classification

Memorization in over-parameterized neural networks could severely hurt generalization in the presence of mislabeled examples. However, mislabeled examples are hard to avoid in extremely large datasets collected with weak supervision. We address this problem by reasoning counterfactually about the loss distribution of examples with uniform random labels had they were trained with the real examples, and use this information to remove noisy examples from the training set. First, we observe that examples with uniform random labels have higher losses when trained with stochastic gradient descent under large learning rates. Then, we propose to model the loss distribution of the counterfactual examples using only the network parameters, which is able to model such examples with remarkable success. Finally, we propose to remove examples whose loss exceeds a certain quantile of the modeled loss distribution. This leads to On-the-fly Data Denoising (ODD), a simple yet effective algorithm that is robust to mislabeled examples, while introducing almost zero computational overhead compared to standard training. ODD is able to achieve state-of-the-art results on a wide range of datasets including real-world ones such as WebVision and Clothing1M.

==> 10_proof_lm1.tex <==
\section{Theory}
Recently, \citep{soudry2017implicit, nacson2018stochastic} proved that with sufficiently small constant learning rate, SGD iterates converge in direction to the max-margin (hard-margin SVM) solution, assuming the training set is linearly separable. Building upon tools from these works, we first show that in the run of SGD, the ratio of the logistic losses of any two training examples $(\vx_i,y_i),(\vx_j,y_j)$ converges to the ratio of the corresponding values $\alpha_i,\alpha_j$ in the optimal solution to the following dual (hard-margin)  SVM program: %Let $\alpha_1,\dots, \alpha_N$ be the optimal values of the dual variables of  the examples; that is, the optimal solution to the dual SVM program 
\begin{equation}
\label{eq:dual}
\begin{split}
\textup{Maximize }&\sum_{i=1}^N\alpha_i-\frac 12\sum_{i=1}^N\sum_{j=1}^N\alpha_i\alpha_jy_iy_j\vx_i^\top \vx_j\\
\textup{s.t. } & \alpha_1,\cdots,\alpha_N\geq 0.
\end{split}
\end{equation}
Specifically, let $\vw_t$ be the $t$-th iterate of SGD with mini-batch\footnote{Technically, we require all mini-batches to have the same size and each example to be selected in exactly one mini-batch in every epoch.} and constant learning rate $\eta$ on the objective (\ref{eqn:obj}) from any initialization $\vw_0$. We show the following lemma:

\begin{lemma}
\label{lm:sgdratio}
In the setting above, for almost all training sets with respect to the Lebesgue measure, for sufficiently small learning rate $\eta$, the ratio of losses of any two examples $(\vx_i,y_i)$ and $(\vx_j,y_j)$ with $\alpha_j>0$ satisfies
\begin{equation}
\lim\limits_{t\rightarrow \infty}\frac{\ell(\vw_t;\vx_i,y_i)}{\ell(\vw_t;\vx_j,y_j)}=\frac{\alpha_i}{\alpha_j}.
\end{equation}
%\lh{Need linear independence. Need every $\alpha_i>0$.}
\end{lemma}

\subsection{A Lemma about SGD Iterates}
In order to prove Lemma \ref{lm:sgdratio}, we will first prove a lemma (Lemma \ref{lm:sgd_max_margin}) about SGD iterates in linear binary classification with the logistic loss. We consider SGD with minibatch and we assume each epoch consists of $K$ iterations each corresponding to a minibatch of size $B=N/K$. We assume the $K$ minibatches in each epoch are disjoint. For $t = 0,1,\cdots$, SGD does the following update:
\begin{equation}
    \vw_{t+1}\gets \vw_t - \eta\sum_{i\in B(t)}\nabla_{\vw}\ell(\vw;\vx_i,y_i)|_{\vw = \vw_t}
\end{equation}
for minibatch $B(t)\subseteq \{1,\cdots,N\}$ with $|B(t)| = B$. 

Our analysis is inspired by \citet{soudry2017implicit} and \citet{nacson2018stochastic}, who showed that when the training set is linearly separable and when the learning rate $\eta$ is sufficiently small, the SGD iterates converge in direction to the hard-margin SVM solution $\hat \vw$, i.e., the optimal solution to the following SVM program (the primal form of (\ref{eq:dual})):
\begin{equation}
    \label{eq:primal}
    \begin{split}
    \text{Minimize }&\frac 12\|\vw\|_2^2,\\
    \text{s.t. }&\forall 1\leq i\leq N, y_i\vw^\top \vx_i\geq 1.
    \end{split}
\end{equation}
By duality, we always have $\hat \vw = \sum_{i=1}^N \alpha_iy_i\vx_i$. By complementary slackness, we have $y_i\hat\vw^\top \vx_i >1\Rightarrow \alpha_i = 0$. Therefore, if we define $S=\{i\in \{1,\cdots,N\}: y_i\hat\vw^\top\vx_i=1\}$ to be the set of indices of the support vectors, we have $\forall i\notin S, \alpha_i = 0$, and thus $\hat\vw = \sum_{i\in S}\alpha_iy_i\vx_i$. This then implies the following equality about the norm of $\hat \vw$:
\begin{equation}
    \|\hat\vw\|_2^2 = \hat\vw^\top \hat\vw = \sum_{i\in S}\alpha_iy_i\hat\vw^\top \vx_i = \sum_{i\in S}\alpha_i = \sum_{i=1}^n\alpha_i.
\end{equation}
Since $\hat\vw$ achieves the maximum normalized margin (margin divided by $\|\vw\|_2$) among all linear classifiers, we have the following claim:
\begin{claim}
\label{claim:margin}
Suppose the training set is linearly separable, i.e., the maximum normalized margin
\begin{equation}
\gamma^*:=\max_{\vw\in\bb R^d, \|\vw\|_2 = 1}\min_{1\leq i\leq N}y_i\vw^\top \vx_i
\end{equation}
is positive. Then $\gamma^* = \left(\sum_{i=1}^N\alpha_i\right)^{-1/2}$.
\end{claim}

\citep{nacson2018stochastic} proved the following lemma showing that, when we run SGD with sufficiently small learning rate, the training loss converges to zero.
\begin{lemma}[Theorem 1 in \citep{nacson2018stochastic}]
\label{nlm:zerothorder}
Suppose the training set is linearly separable. Define $X\in \bb R^{d\times N}$ such that the $i$-th column of $X$ is $y_i\vx_i$. Suppose
\begin{equation}
\label{eq:small_rate}
    \eta < \min\left\{\frac 1{2K\beta\sigma_{\max}^2(X)}, \frac {\gamma^*}{2\beta\sigma^3_{\max}(X)(K+\sigma_{\max}(X)/\gamma^*)}\right\},
\end{equation}
where $\gamma^*=\left(\sum_{i=1}^N\alpha_i\right)^{-1/2}$ is the maximum normalized margin and $\beta = \frac 14$ is the smoothness coefficient of the logistic loss $\mathrm{loss}(z)=\ln(1+\exp(-z))$. Then, $\forall 1\leq i\leq N$,
\begin{equation}
\vw_t^\top \vx_i\rightarrow +\infty \text{ as } t\rightarrow +\infty.
\end{equation}
\end{lemma}
Lemma \ref{nlm:zerothorder} implies the following corollary about the asymptotic behavior of the logistic loss and its gradient:
\begin{corollary}
\label{cor:asymptotic}
Suppose the training set is linearly separable and the learning rate $\eta$ satisfies (\ref{eq:small_rate}). Then, $\forall 1\leq i\leq N$, as $t\rightarrow +\infty$,
\begin{align}
    \frac{\ell(\vw_t;\vx_i,y_i)}{\exp(-y_i\vw_t^\top \vx_i)} = & 1 + o(1),\\
    \frac{\nabla_\vw \ell(\vw;\vx_i,y_i)|_{\vw = \vw_t}}{\exp(-y_i\vw_t^\top \vx_i)} = &  -(1+o(1))y_i\vx_i.
\end{align}
\end{corollary}
The following claim is the ``converse'' of complementary slackness:
\begin{claim}
\label{claim:zeromeasure}
Suppose the data dimension is larger than the size of the training set, i.e., $d > N$. Then, for almost all training sets with respect to the Lebesgue measure, $(\vx_i)_{1\leq i\leq N}$ are linearly independent and $\forall i\in S,\alpha_i>0$.
\end{claim}
\begin{proof}
For any fixed $i$, almost surely with respect to the Lebesgue measure, $\vx_i$ is not in the subspace spanned by $(\vx_j)_{j\neq i}$ because the subspace has dimension less than $d$ and is independent of $\vx_i$. This implies $(\vx_i)_{1\leq i\leq N}$ are linearly independent almost surely. If we condition on $(x_i)_{1\leq i\leq N}$ being linearly independent, when $i\in S$, i.e., $\vx_i$ is a support vector, almost surely $\alpha_i>0$ because otherwise $\vx_i$ is on the supporting hyper-plane determined by the other support vectors, which again has dimension less than $d$ and is independent of $\vx_i$.
\end{proof}
% 
% 
%
%Since we assume we are in the over-parametrized regime, i.e., $d>N$, we know the $\vx_i$ in the training set are linearly independent almost surely with respect to the Lebesgue measure, and in this case, the training set is linearly separable.
We are now ready to state and prove the following key lemma about SGD iterates.
\begin{lemma}
\label{lm:sgd_max_margin}
% Suppose we have $N$ training examples, $(x_1,y_1),(x_2,y_2),\cdots,(x_N,y_N)\in\bb R^d\times\{\pm 1\}$. Assume $x_1,x_2,\cdots,x_N$ are linearly independent. Suppose we train a linear model $f_w(x)=w^\top x$ using Stochastic Gradient Descent on the objective $\sum_{i=1}^N\ell(y_if_w(x_i))$ using constant learning rate $\eta$, where the loss function $\ell(\cdot)$ is the logistic loss $\ell(z)=\ln(1+\exp(-z))$, and get iterate $w_t$ after iteration $t$. 
Assume $(\vx_i)_{1\leq i\leq N}$ are linearly independent and $\forall i\in S,\alpha_i>0$. Assume the learning rate $\eta$ satisfies (\ref{eq:small_rate}). %, and in each epoch every training example is selected in exactly one minibatch.  
% We define $\gamma(w)$ to be the margin of $w$ on the training set: $\gamma(w)=\min_{1\leq i\leq N}y_if_w(x_i)$, and $\hat w$ to be the max-margin solution: $\hat w = \argmin\{\|w\|_2:\gamma(w)\geq 1\}$. 
%Define $X=[y_1x_1,y_2x_2,\cdots,y_Nx_N]\in\bb R^{d\times N}$. 
Define $\theta:=\min_{i\notin S}y_i\hat \vw^\top \vx_i>1$. Define $P_Y:\bb R^d\rightarrow Y$ to be the orthogonal projection operator onto the subspace spanned by support vectors $Y:=\mathrm{span}(\{\vx_i:i\in S\})$. Then there exists $\tilde \vw\in Y$ such that $\forall i\in S,\exp(-y_i\tilde \vw^\top \vx_i)=\frac{\alpha_i}\eta$ and for any initialization $\vw_0\in\bb R^d$,
\begin{equation}
    \lim\limits_{t\rightarrow +\infty}\left\|P_Y(\vw_t)-\ln\left(\frac tK\right)\hat \vw-\tilde \vw\right\|_2=0.
\end{equation}
%where $\hat w = X\bm\alpha$.

% Assume the examples are linearly separable with max-margin solution $\hat w\neq \mathbf 0$ and corresponding dual solutions $\alpha_1,\alpha_2,\cdots,\alpha_m\in\bb R_{> 0}$ satisfying $\sum_{i=1}^m\alpha_iy_ix_i=\hat w$. Note that here we assume $\alpha_i>0$ for every $i$, which implies every example $(x_i,y_i)$ is a ``support vector'', i.e., $y_i\hat w^\top x_i=1$. Let $\ell(w;x,y)=\ell(yw^\top x)=\ln(1+\exp(-yw^\top x))$ be the Logistic loss. Suppose $w_0\in\bb R^d$ is any initialized weight. For any $t\in\bb N^*$, at time step $t$, we update $w_{t-1}$ to $w_t$ using Stochastic Gradient Descent with batch $B(t)\subseteq \{1,2,\cdots,m\}$:
% \begin{equation}
% \label{eq:sgd_update}
%     w_t=w_{t-1} - \eta\sum\limits_{i\in B(t)}\nabla_w\ell(w_{t-1};x_i,y_i).
% \end{equation}
% Here $\eta\in\bb R_{>0}$ is the learning rate. Suppose each epoch has $K$ iterations, and for every $p\in\bb N^*$, $B(pK-K+1),B(pK-K+2),\cdots,B(pK)$ form a partition of $\{1,2,\cdots,m\}$. Assume the learning rate satisfies
% \begin{equation*}
%     \eta < \min\{\frac 1{2K\beta\sigma_{\max}^2}, \frac r{2\beta\sigma^3_{\max}(K+r ^{-1}\sigma_{\max})}\},
% \end{equation*}
% where $r = \frac 1{\|\hat w\|}$, $\beta$ is the smoothness coefficient of the Logistic loss and $\sigma_{\max}$ is the maximum singular value of the matrix $[x_1,x_2,\cdots,x_m]\in\bb R^{d\times m}$.

% Then, there exist $\tilde w\in\bb R^d$ satisfying $\forall i,\exp(-y_i\tilde w^\top x_i)=\frac{\alpha_i}{\eta}$ and
% \begin{equation*}
%     \lim\limits_{t\rightarrow +\infty}\left\|w_t-\ln\left(\frac tK\right)\hat w-\tilde w\right\|=0
% \end{equation*}
\end{lemma}

\begin{proof}
% Since $x_1,x_2,\cdots,x_N$ are linearly independent, $X$ has full column rank and $X^\top X$ is invertible. This proves the existence and uniqueness of $\bm\alpha$. Let's now focus on the case where every $\alpha_i$ is non-negative and the learning rate satisfies (\ref{eq:small_rate}).

% Consider the following hard-margin SVM problem:
% \begin{align*}
%     \text{Minimize }&\frac 12\|w\|_2^2,\\
%     \text{s.t. }&\forall 1\leq i\leq N, y_iw^\top x_i\geq 1.
% \end{align*}
% By definition, $X^\top \hat w=X^\top X\bm\alpha = (1,1,\cdots,1)^\top$. Therefore, $\hat w$ is a feasible solution to the above optimization problem with objective value $\frac 12\|\hat w\|_2^2=\frac 12\hat w^\top \hat w=\frac 12\bm\alpha^\top X^\top X\bm\alpha=\frac 12\bm\alpha^\top (1,1,\cdots,1)^\top=\frac 12\sum_{i=1}^N\alpha_i$. Moreover, $\bm\alpha$ is a feasible solution to the dual:
% \begin{align*}
%     \text{Maximize }&\sum_{i=1}^N\alpha_i-\frac 12\sum_{i=1}^N\sum_{j=1}^N\alpha_i\alpha_jy_iy_jx_i^\top x_j,\\
%     \text{s.t. }&\forall 1\leq i\leq N,\alpha_i\geq 0,
% \end{align*}
% with objective value $\sum_{i=1}^N\alpha_i-\frac 12\bm\alpha^\top X^\top X\bm\alpha=\sum_{i=1}^N\alpha_i-\frac 12\bm\alpha^\top (1,1,\cdots,1)^\top=\frac 12\sum_{i=1}^N\alpha_i$. Therefore, $\hat w$ is the global optimum of the primal and $\bm\alpha$ is the global optimum of the dual. %By complementary slackness, every $\alpha_i$ being positive means every training example being a support vector. 
% Moreover, $\gamma^* = \left(\sum_{i=1}^N\alpha_i\right)^{-1/2} = \|\hat w\|_2^{-1}$ equals to the maximum normalized margin $\max_{\|w\|_2 = 1}\min_{1\leq i\leq N}y_iw^\top x_i$.
Note that we assumed $\vx_1,\vx_2,\cdots,\vx_N$ to be linearly independent, so there exists a unique $\tilde \vw\in Y$ satisfying $\forall i\in S,\exp(-y_i\tilde \vw^\top \vx_i)=\frac{\alpha_i}{\eta}$. The rest is to show that $\lim\limits_{t\rightarrow +\infty}\|P_Y(\vw_t)-\ln(\frac tK)\hat \vw-\tilde \vw\|_2=0$.

Let's first show that we can assume $\vw_0\in\Span(\vx_1,\vx_2,\cdots,\vx_N)$ without loss of generality. Otherwise, say $\vw_0=\bar \vw+\vw_0'$ where $\vw_0'\in\Span(\vx_1,\vx_2,\cdots,\vx_N)$ and $\bar \vw \perp \Span(\vx_1,\vx_2,\cdots,\vx_N)$. Then, the SGD update rule ensures that for every $t$, $\vw_t=\bar \vw + \vw_t'$ with $\vw_t'\in\Span(\vx_1,\vx_2,\cdots,\vx_N)$, so $P_Y(\vw_t)=P_Y(\vw_t')$. Moreover, the sequence $\vw_t'$ can be generated by SGD with initialization $\vw_0'$. Therefore, we only need to consider initialization $\vw_0'$ and get a proof for $\vw_0$ automatically.
%If we could prove the lemma for $w_0'$, i.e., there exists $\tilde w\in\bb R^d$ satisfying $\forall i,\exp(-y_i\tilde w^\top x_i)=\frac{\alpha_i}{\eta}$ and $\lim\limits_{t\rightarrow +\infty}\|P_Y(w_t')-\ln(\frac tK)\hat w - \tilde w\|_2=0$, then taking $\tilde w=\tilde w'+w^\perp$ yields a proof for $w_0$.

Now we assume $\vw_0\in\Span(\vx_1,\vx_2,\cdots,\vx_N)$ without loss of generality, and consequently $\vw_t\in\Span(\vx_1,\vx_2,\cdots,\vx_N)$ for every $t\geq 0$. 
Note that we can also assume $y_i=1$ for $1\leq i\leq N$ without loss of generality by replacing $y_i\vx_i$ by a new $\vx_i$. Recall $B(u)$ is the set of indices of training examples selected in the mini-batch corresponding to the $u$-th iteration. By Lemma 5 in \cite{nacson2018stochastic}, we know that $\ln(\frac tK)\hat \vw=K\sum\limits_{u=1}^{t-1}\frac 1u\sum\limits_{i\in S\cap B(u)}\alpha_i\vx_i-\gamma \hat \vw+o(1)$ as $t\rightarrow +\infty$, where $\gamma$ is the Euler-Mascheroni constant. %where $\|m_4(t)\|=o(t^{-0.5})$. 
Therefore, we only need to show that $\lim\limits_{t\rightarrow +\infty}\|P_Y(\vr(t))\|_2=0$, where 
\begin{equation}
    \vr(t)=\vw_t-K\sum\limits_{u=1}^{t-1}\frac 1u\sum\limits_{i\in S\cap B(u)}\alpha_i\vx_i+\gamma\hat \vw-\tilde \vw\in\mathrm{span}(\vx_1,\cdots,\vx_N).
\end{equation}

We will use the following results proved in \citep{nacson2018stochastic}:
\begin{lemma}[Theorem 2 in \citep{nacson2018stochastic}]
\label{nlm:direction}
$\vw_t = \ln(\frac tK)\hat \vw + O(1)$ as $t\rightarrow +\infty$.
\end{lemma}
\begin{lemma}[in Section B.1 of \citep{nacson2018stochastic}]
\label{nlm:series}
$\sum_{t=1}^{+\infty}\|\vr(t+1)-\vr(t)\|_2^2<\infty$.
\end{lemma}
\begin{lemma}[Lemma 6 in \cite{nacson2018stochastic}]
\label{nlm:dot}
There exist $c_1,\delta>0$ such that for all $t\in\bb N^*$, it holds that
\begin{equation}
    (\vr(t+1)-\vr(t))^\top \vr(t)\leq c_1t^{-1-\delta}.
\end{equation}
\end{lemma}
Lemma \ref{nlm:series} and Lemma \ref{nlm:dot} imply that $\forall \varepsilon>0$, there exists $t_1\in\bb N^*$ such that $\forall t',t''\in\bb N^*\text{ with }t''>t'\geq t_1$,
\begin{align}
&\|\vr(t'')\|_2^2-\|\vr(t')\|_2^2\nonumber \\
   =&\sum\limits_{t=t'}^{t''-1}(\|\vr(t+1)\|_2^2-\|\vr(t)\|_2^2)\nonumber \\
  =&\sum\limits_{t=t'}^{t''-1}(\|\vr(t+1)-\vr(t)\|_2^2+2(\vr(t+1)-\vr(t))^\top \vr(t))\nonumber \\
  \leq &\sum\limits_{t=t'}^{t''-1}\|\vr(t+1)-\vr(t)\|_2^2+2c_1\sum\limits_{t=t'}^{t''-1}t^{-1-\delta}\nonumber \\
  \leq & \varepsilon.  \label{eq:partialsum}
\end{align}
Define subspace $Z:=\{\vx\in\mathrm{span}(\vx_1,\cdots,\vx_N): \vx \perp Y\}$ and let $P_Z$ be the orthogonal projection operator onto $Z$. We show that $\sum_{t = 1}^{+\infty}\|P_Z(\vr(t+1))-P_Z(\vr(t))\|_2 < +\infty$, and thus there exists $\vr^\perp\in Z$ such that $P_Z(\vr(t))\rightarrow \vr^\perp$ as $t\rightarrow +\infty$. Note that $\vr(t)-\vw_t\in Y$ and $Y$ is orthogonal to $Z$, so we have $\|P_Z(\vr(t+1))-P_Z(\vr(t))\|_2 = \|P_Z(\vw_{t+1})-P_Z(\vw_t)\|_2$. By the SGD update rule, we have $\vw_{t+1}-\vw_t = \eta\sum_{i\in B(t)}\nabla_{\vw} \ell(\vw;\vx_i,y_i)|_{\vw = \vw_t}$. When $i\in S$, we know that $\nabla_{\vw} \ell(\vw;\vx_i,y_i)|_{\vw = \vw_t}$, as a scalar multiple of $\vx_i$, is in $Y$, contributing zero to the orthogonal projection onto $Z$. Therefore, $\|P_Z(\vw_{t+1})-P_Z(\vw_t)\|_2\leq \eta\sum_{i\in B(t)\backslash S}\|\nabla_{\vw}\ell(\vw;\vx_i,y_i)|_{\vw=\vw_t}\|_2 \leq \eta\sum_{i\notin S}\|\nabla_{\vw}\ell(\vw;\vx_i,y_i)|_{\vw=\vw_t}\|_2$. According to Lemma \ref{nlm:direction}, as $t\rightarrow +\infty$, $\vw_t = \ln(\frac tK)\hat \vw + O(1)$, so for every $i\notin S$, $\exp(-\vw_t^\top \vx_i) = O(\exp(-\ln(\frac tK)\hat \vw^\top \vx_i))  = O(\exp(-\ln(\frac tK)\theta)) = O((\frac{K}{t})^\theta) = O(t^{-\theta})$, where we used the fact that $\hat\vw^\top \vx_i\geq\theta$. Therefore, according to Corollary \ref{cor:asymptotic}, we have $\forall i\notin S, \|\nabla_{\vw}\ell(\vw;\vx_i,y_i)|_{\vw=\vw_t}\|_2 = O(t^{-\theta})$ and the desired
\begin{equation}
\sum_{t = 1}^{+\infty}\|P_Z(\vr(t+1))-P_Z(\vr(t))\|_2 = \sum_{t = 1}^{+\infty} \|P_Z(\vw_{t+1})-P_Z(\vw_t)\|_2 \leq \eta N \sum_{t = 1}^{+\infty} t^{-\theta} < +\infty. 
\end{equation}
Now we have proved that $P_Z(\vr(t))$ converges as $t\rightarrow +\infty$. Let $\vr^\perp$ be the limit. Since the squred $L_2$ norm is continuous, $\forall \varepsilon > 0$, there exists $t_0\in\bb N^*$ such that $\forall t\geq t_0$, it holds that 
\begin{equation}
\label{eq:pzlimit}
|\|P_Z(\vr(t))\|_2^2-\|\vr^\perp\|_2^2|\leq \varepsilon.
\end{equation}

% In Section B.1, \citet{nacson2018stochastic} showed that $\sum_{t=0}^{+\infty}\|\vr(t+1)-\vr(t)\|_2^2<\infty$. Lemma 6 in \cite{nacson2018stochastic} showed that there exist $c_1,\delta>0$ such that for all $t\in\bb N^*$, it holds that
% \begin{equation*}
%     (\vr(t+1)-\vr(t))^\top \vr(t)\leq c_1t^{-1-\delta}.
% \end{equation*}
% Therefore, we can find $t_1\in\bb N^*$ such that $\forall t',t''\in\bb N^*\text{ with }t''>t'\geq t_1$,
% \begin{align}
% &\|\vr(t'')\|_2^2-\|\vr(t')\|_2^2\nonumber \\
%   =&\sum\limits_{t=t'}^{t''-1}(\|\vr(t+1)\|_2^2-\|\vr(t)\|_2^2)\nonumber \\
%   =&\sum\limits_{t=t'}^{t''-1}(\|\vr(t+1)-\vr(t)\|_2^2+2(\vr(t+1)-\vr(t))^\top \vr(t))\nonumber \\
%   \leq &\sum\limits_{t=t'}^{t''-1}\|\vr(t+1)-\vr(t)\|_2^2+2c_1\sum\limits_{t=t'}^{t''-1}t^{-1-\delta}\nonumber \\
%   \leq & \varepsilon. 
% \end{align}
Now we use the following lemma proved later in Section \ref{sec:helper}.
\begin{lemma}
\label{lm:helper}
$\forall \varepsilon > 0$, there exist $c_2>0$ and $t_2\in\bb N^*$ such that for all $t\geq t_2$ with $\|P_Y(\vr(t))\|_2\geq \varepsilon$, there exists $t'\in\bb N^*$ with $t\leq t'<t+2K$ satisfying $(\vr(t'+1)-\vr(t'))^\top \vr(t')\leq -c_2t^{-1}$. 
\end{lemma}


Assume for the sake of contradiction that $\|P_Y(\vr(t))\|_2\geq\varepsilon$ for all $t\geq t_{\max}:=\max\{t_0,t_1,t_2\}$ ($t_2$ as in Lemma \ref{lm:helper}). Then 
\begin{align}
&\sum\limits_{t\geq t_{\max}}(\|\vr(t+1)\|_2^2-\|\vr(t)\|_2^2)\nonumber \\
=&\sum\limits_{t\geq t_{\max}}\|\vr(t+1)-\vr(t)\|_2^2+2\sum\limits_{t\geq t_{\max}}(\vr(t+1)-\vr(t))^\top \vr(t)\nonumber \\
\leq &\varepsilon+2c_1\sum\limits_{t\geq t_{\max}}t^{-1-\delta}-2c_2\sum\limits_{ \genfrac{}{}{0pt}{2}{t\geq t_{\max}}{t\text{ is a multiple of }2K}}t^{-1}\nonumber \\
=&-\infty,
\end{align}
a contradiction. Therefore, there exists $t_3\geq t_{\max}$ with $\|P_Y(\vr(t_3))\|_2\leq \varepsilon$. Now for any $t\geq t_3$, we have 
\begin{align}
&\|P_Y(\vr(t))\|_2^2\nonumber \\
= & \|P_Y(\vr(t_3))\|_2^2 + (\|P_Y(\vr(t))\|_2^2-\|P_Y(\vr(t_3))\|_2^2)\nonumber \\
= & \|P_Y(\vr(t_3))\|_2^2 + (\|\vr(t)\|_2^2-\|\vr(t_3)\|_2^2) - (\|P_Z(\vr(t))\|_2^2-\|P_Z(\vr(t_3))\|_2^2)\nonumber \\
= & \|P_Y(\vr(t_3))\|_2^2 + (\|\vr(t)\|_2^2-\|\vr(t_3)\|_2^2) - (\|P_Z(\vr(t))\|_2^2 - \|\vr^\perp\|_2^2) -(\|\vr^\perp\|_2^2 - \|P_Z(\vr(t_3))\|_2^2)\nonumber \\
\leq & \varepsilon^2+\varepsilon + \varepsilon + \varepsilon,
\end{align}
according to (\ref{eq:pzlimit}) and (\ref{eq:partialsum}). By the arbitrariness of $\varepsilon>0$, we have proved $\lim\limits_{t\rightarrow +\infty}\|P_Y(\vr(t))\|_2=0$.
\end{proof}
\subsection{Proof of Lemma \ref{lm:helper}}
\label{sec:helper}
We need a technical lemma from \citep{nacson2018stochastic} in order to prove Lemma \ref{lm:helper}. In Eq.\ 46 in Section B.2 of \citep{nacson2018stochastic}, $(\vr(t+1)-\vr(t))^\top \vr(t)$ is decomposed into the sum of two parts:
\begin{align}
    & (\vr(t+1)-\vr(t))^\top \vr(t)\nonumber \\
    = & \left[-\eta \sum_{i\in B(t)\backslash S}\vr(t)^\top \nabla_\vw\ell(\vw;\vx_i,y_i)|_{\vw = \vw_t}\right]\nonumber \\
    & + \left[-\eta \sum_{i\in S\cap B(t)}\vr(t)^\top \nabla_\vw\ell(\vw;\vx_i,y_i)|_{\vw = \vw_t} - \frac Kt \sum_{i\in S\cap B(t)}\alpha_i\vx_i^\top \vr(t)\right].
\end{align}
\citep{nacson2018stochastic} showed that, as $t\rightarrow +\infty$, the first part is upper bounded by $O(t^{-1-\delta_1})$ for some $\delta_1>0$, while the second part is upper bounded by $\sum_{i\in S\cap B(t)}\alpha_i\frac K{t}(\gamma_i(t)\exp(\tilde m_i(t)-\vx_i^\top \vr(t))-1)\vx_i^\top \vr(t)$, which is again upper bounded by $O(t^{-1-\delta_2})$ for some $\delta_2>0$. Specifically, we have the following lemma:
\begin{lemma}[in Section B.2 of \citep{nacson2018stochastic}]
\label{lm:technical}
There exists $\delta_1>0$ such that as $t\rightarrow +\infty$, 
\begin{equation}
\label{eq:decomposition}
    (\vr(t+1)-\vr(t))^\top \vr(t)\leq \sum\limits_{i\in S\cap B(t)}\alpha_i\frac K{t}(\gamma_i(t)\exp(\tilde m_i(t)-\vx_i^\top \vr(t))-1)\vx_i^\top \vr(t) + O(t^{-1-\delta_1}),
\end{equation}
where $\tilde m_i(t)\rightarrow 0$ and $\gamma_i(t)\rightarrow 1$ as $t\rightarrow +\infty$. Moreover, there exists $\delta_2>0$ such that as $t\rightarrow +\infty$,
\begin{equation}
    \max_{i\in S\cap B(t)}\alpha_i\frac K{t}(\gamma_i(t)\exp(\tilde m_i(t)-\vx_i^\top \vr(t))-1)\vx_i^\top \vr(t) = O(t^{-1-\delta_2}).
\end{equation}
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lm:helper}]
Based on Lemma \ref{lm:technical}, we only need to prove that there exist $c_2>0$ and $t_2\in\bb N^*$ such that for all $t\geq t_2$ with $\|P_Y(\vr(t))\|_2\geq\varepsilon$, there exist $t'\in\bb N^*$ with $t\leq t' < t+2K$ and $i_1\in S\cap B(t')$ satisfying
\begin{equation}
    \label{eq:negative}
    \alpha_{i_1}\frac K{t'}(\gamma_{i_1}(t')\exp(\tilde m_{i_1}(t')-\vx_{i_1}^\top \vr(t'))-1)\vx_{i_1}^\top \vr(t') \leq -c_2(t')^{-1}.
\end{equation}

Define $\bar X\in\bb R^{d\times |S|}$ so that each column of $\bar X$ corresponds to an $\vx_i$ for $i\in S$. We assumed that $\vx_1,\cdots,\vx_N$ are linearly independent, so $\bar X^\top$ has a positive minimum singular value $\sigma_{\min}:=\min_{\vr\in Y:\|\vr\|_2=1}\|\bar X^\top \vr\|_2>0$ and thus
$\|\bar X^\top P_Y(\vr(t))\|_2\geq \sigma_{\min}\|P_Y(\vr(t))\|_2\geq \sigma_{\min}\varepsilon$.
Therefore, there exists $i_1\in S$ such that 
$|\vx_{i_1}^\top \vr(t)| = |\vx_{i_1}^\top P_Y(\vr(t))|\geq \varepsilon_1:=\frac{\sigma_{\min} \varepsilon}{\sqrt N}$.
According to Lemma \ref{nlm:series}, by picking $t_2$ sufficiently large, we can ensure that for every $t\geq t_2$, it holds that $\|\vr(t+1)-\vr(t)\|_2\leq \frac{\varepsilon_1}{4K(\max_{1\leq i\leq N}\|\vx_i\|_2)}$. Then, $\forall t'\in\bb N^*$ with $t\leq t'<t+2K$, we have $|\vx_{i_1}^\top \vr(t')|\geq |\vx_{i_1}^\top \vr(t)|-|\vx_{i_1}^\top (\vr(t)-\vr(t'))|\geq \varepsilon_1-\|\vx_{i_1}\|_2\|\vr(t)-\vr(t')\|_2\geq \frac{\varepsilon_1} 2$. Pick $t'$ so that $i_1\in B(t')$. 
%In Section B.2, \citet{nacson2018stochastic} showed that
% \begin{equation}
%     (\vr(t'+1)-\vr(t'))^\top \vr(t')\leq \sum\limits_{i\in S\cap B(t')}\alpha_i\frac K{t'}(\gamma_i(t')\exp(\tilde m_i(t')-\vx_i^\top \vr(t'))-1)\vx_i^\top \vr(t') + O(t^{-1-\delta})
% \end{equation}
% as long as we pick $t_2$ sufficiently large, where $\tilde m_i(t)\rightarrow 0$ and $\gamma_i(t)\rightarrow 1$ as $t\rightarrow +\infty$. In Section B.2, \citet{nacson2018stochastic} also showed that there exist $c',\delta'\in\bb R_{>0}$ independent of $t,t'$ such that $\forall 1\leq i\leq N$
% \begin{equation}
% \label{eq:positive}
%     \alpha_i\frac K{t'}(\gamma_i(t')\exp(\tilde m_i(t')-\vx_i^\top \vr(t'))-1)\vx_i^\top \vr(t')\leq c'(t')^{-1-\delta'}\leq c't^{-1-\delta'}.
% \end{equation}
% Now we show that there exists $c_2'\in\bb R_{>0}$ independent of $t,t'$ such that 
% \begin{equation}
% \label{eq:negative}
%     \alpha_{i_1}\frac K{t'}(\gamma_{i_1}(t')\exp(\tilde m_{i_1}(t')-\vx_{i_1}^\top \vr(t'))-1)\vx_{i_1}^\top \vr(t')\leq -c_2'(t')^{-1}\leq -c_2'(t+2K)^{-1}.
% \end{equation}

When $\vx_{i_1}^\top \vr(t')\geq \frac{\varepsilon_1}{2}$, as long as we pick $t_2$ sufficiently large, we can make sure that $\gamma_{i_1}(t')\exp(\tilde m_{i_1}(t')-\vx_{i_1}^\top \vr(t'))-1\leq \exp(-\frac{\varepsilon_1}{4})-1$, so the left hand side of (\ref{eq:negative}) is upper bounded by $-\alpha_{i_1}\frac K{t'}\frac{\varepsilon_1}{2}(1-\exp(-\frac{\varepsilon_1}{4}))$. Similarly, when $\vx_{i_1}^\top \vr(t')\leq -\frac{\varepsilon_1}{2}$, as long as we pick $t_2$ sufficiently large, we can make sure that $\gamma_{i_1}(t')\exp(\tilde m_{i_1}(t')-\vx_{i_1}^\top \vr(t'))-1\geq \exp(\frac{\varepsilon_1}{4})-1$, so the left hand side of (\ref{eq:negative}) is again upper bounded by $-\alpha_{i_1}\frac K{t'}\frac{\varepsilon_1}{2}(\exp(\frac{\varepsilon_1}{4})-1)\leq -\alpha_{i_1}\frac K{t'}\frac{\varepsilon_1}{2}(1-\exp(-\frac{\varepsilon_1}{4}))$. Therefore, we can choose $c_2'=(\min_{i\in S}\alpha_{i})K\varepsilon_1(1-\exp(-\varepsilon_1/4))/2$ to make (\ref{eq:negative}) hold true.
% 
% Combining (\ref{eq:positive}) and (\ref{eq:negative}) with (\ref{eq:decomposition}), we know
% \begin{align*}
%     & (\vr(t'+1)-\vr(t'))^\top \vr(t')\\
%     \leq & |S\cap B(t')|c't^{-1-\delta'}-c_2'(t+2K)^{-1} + O(t^{-1-\delta})\\
%     \leq & c'Nt^{-1-\delta'}-c_2'(t+2K)^{-1} + O(t^{-1-\delta}).
% \end{align*}
% Now as long as we pick $t_2$ sufficiently large, we know there exists $c_2>0$ independent of $t,t'$ such that $(\vr(t'+1)-\vr(t'))^\top \vr(t')\leq -c_2t^{-1}$.
\end{proof}
\subsection{Proof of Lemma \ref{lm:sgdratio}}
Lemma \ref{lm:sgdratio} is a direct corollary of Claim \ref{claim:zeromeasure} and the following lemma.
\begin{lemma}
\label{lm:sgdratio_}
In the setting of Lemma \ref{lm:sgd_max_margin}, $\forall 1\leq i,j\leq N$, if $\alpha_j>0$, we have 
\begin{equation}
\lim\limits_{t\rightarrow \infty}\frac{\ell(\vw_t;\vx_i,y_i)}{\ell(\vw_t;\vx_j,y_j)}=\frac{\alpha_i}{\alpha_j}.
\end{equation}
\end{lemma}
\begin{proof}
By Lemma \ref{lm:sgd_max_margin}, we have $P_Y(\vw_t)=\ln(\frac tK)\hat \vw + \tilde \vw + o(1)$. According to Lemma \ref{nlm:direction} (Theorem 2 in \citep{nacson2018stochastic}) we also have $\vw_t = \ln(\frac tK)\hat \vw + O(1)$.

By Corollary \ref{cor:asymptotic}, we have $\lim\limits_{t\rightarrow +\infty}\frac{\ell(\vw_t;\vx_i,y_i)}{\exp(-y_i\vw_t^\top \vx_i)}=1$. %\lh{TO DO: make slight changes to adapt to the statement of Lemma 1.} 
Therefore, we only need to show that $\lim\limits_{t\rightarrow +\infty}\frac{\exp(-y_i\vw_t^\top \vx_i)}{\exp(-y_j\vw_t^\top \vx_j)}=\frac{\alpha_i}{\alpha_j}$.
%According to Lemma \ref{lm:sgd_max_margin}, we have $w_t=\ln\left(\frac tK\right)\hat w+\tilde w + o(1)$. Note that $y_i\hat w^\top x_i=1,\exp(-y_i\tilde w^\top x_i)=\frac{\alpha_i}{\eta}$, we have

Let's first assume $\alpha_i>0$. Since we also assumed $\alpha_j>0$, so by complementary slackness, $i$ and $j$ are both in $S$. In this case $\vx_i$ and $\vx_j$ are both in subspace $Y$, so they are both orthogonal to $\vw_t-P_Y(\vw_t)$. Therefore,
\allowdisplaybreaks
\begin{align}
    &\lim\limits_{t\rightarrow +\infty}\frac{\exp(-y_i\vw_t^\top \vx_i)}{\exp(-y_j\vw_t^\top \vx_j)}\nonumber \\
    = &\lim\limits_{t\rightarrow +\infty}\frac{\exp(-y_iP_Y(\vw_t)^\top \vx_i)}{\exp(-y_jP_Y(\vw_t)^\top \vx_j)}\nonumber \\
    =&\lim\limits_{t\rightarrow +\infty}\frac{\exp(-y_i\ln(\frac tK)\hat \vw^\top \vx_i)\exp(-y_i\tilde \vw^\top \vx_i)\exp(o(1))}{\exp(-y_j\ln(\frac tK)\hat \vw^\top \vx_j)\exp(-y_j\tilde \vw^\top \vx_j)\exp(o(1))}\nonumber \\
    =&\lim\limits_{t\rightarrow +\infty}\frac{(\frac tK)^{-1}\cdot \frac{\alpha_i}{\eta}\exp(o(1))}{(\frac tK)^{-1}\cdot \frac{\alpha_j}{\eta}\exp(o(1))}\nonumber \\
    =&\lim\limits_{t\rightarrow +\infty}\frac{\alpha_i\exp(o(1))}{\alpha_j\exp(o(1))}\nonumber \\
    =&\frac {\alpha_i}{\alpha_j}.
\end{align}

When $\alpha_i=0$, we have $i\notin S$ but $j\in S$, and thus
\allowdisplaybreaks
\begin{align}
    &\lim\limits_{t\rightarrow +\infty}\frac{\exp(-y_i\vw_t^\top \vx_i)}{\exp(-y_j\vw_t^\top \vx_j)}\nonumber \\
    =&\lim\limits_{t\rightarrow +\infty}\frac{\exp(-y_i\ln(\frac tK)\hat \vw^\top \vx_i)\exp(O(1))}{\exp(-y_j\ln(\frac tK)\hat \vw^\top \vx_j)\exp(O(1))}\nonumber \\
    =&\lim\limits_{t\rightarrow +\infty}\frac{O((\frac tK)^{-\theta})}{\Theta((\frac tK)^{-1})}\nonumber \\
    =&\lim\limits_{t\rightarrow +\infty}O(t^{1-\theta})\nonumber \\
    =&0\nonumber \\
    =&\frac{\alpha_i}{\alpha_j}.
\end{align}
\end{proof}


==> 11_proof_thm2.tex <==
\section{Proof of Theorem \ref{thm:loss_separation_linear}}
\label{sec:proof_loss_separation_linear}
\begin{theorem}
\label{thm:loss_separation_linear_re}
Suppose we have $N$ training examples $(\vx_i,y_i)\in\bb R^d\times\{\pm 1\}$  generated by the synthetic model described in Section \ref{sec:theory}, where $n<N/2$ of them are mislabeled and $m = N-n$ of them are clean. 
%Suppose we train a linear classifier $f_w(x)=w^\top x$ using Stochastic Gradient Descent on the objective $\sum_{i=1}^N\ell(y_if_w(x_i))$ using constant learning rate $\eta$, where the loss function $\ell(\cdot)$ is the logistic loss $\ell(z)=\ln(1+\exp(-z))$, and get iterate $w_t$ after iteration $t$. 
Assume each epoch consists of $K$ iterations each corresponding to a minibatch of size $N/K$, and in each epoch every training example is selected in exactly one minibatch. Then, for $\eta = O\left(\left ((N+\lambda^2)\left(mn/\lambda^2 + N + K\sqrt{mn/\lambda^2 + N}\right)\right)^{-1}\right), d=\Omega\left(\left(\frac{N(m+\lambda^2)}{\min\{2n+\lambda^2,m-n\}}\right)^2\log (N/\delta)\right)$, and any initialization $\vw_0$, with  probability at least $1-\delta$ over the randomness of the training set,  there exists $T>0$ such that for all $t>T$, it holds that 
\begin{equation}
    \min_{i:(\vx_i,y_i)\text{ is mislabeled}}\ell(\vw_t;\vx_i,y_i)>\max_{j:(\vx_j,y_j)\text{ is clean}}\ell(\vw_t;\vx_j,y_j).
\end{equation}
\end{theorem}
Before proving Theorem \ref{thm:loss_separation_linear_re}, we first prove the following lemma.
\begin{lemma}
\label{lm:mislabeleddual}
In the setting of Theorem \ref{thm:loss_separation_linear_re}, with probability at least $1-\delta$, the following are true:
\begin{enumerate}
	\item If we define $X = [y_1\vx_1,y_2\vx_2,\cdots,y_N\vx_N]\in\bb R^{d\times N}$, $X$ has full column rank and $\sigma_{\max}(X)\leq \sqrt{N+2\lambda ^2}$;
	\item There exists $\bm\alpha = (\alpha_1,\alpha_2,
	\cdots,\alpha_N)^\top \in\bb R_{>0}^N$ such that $X^\top X\bm\alpha=(1,1,\cdots,1)^\top$;
	\item $\min_{i: (\vx_i,y_i)\text{ is mislabeled}}\alpha_i>\max_{j: (\vx_j,y_j)\text{ is clean}}\alpha_i$;
	\item $\frac 12\sqrt{\frac{4mn + \lambda^2N}{\lambda^2(N+\lambda^2)}}\leq \sqrt{\sum_{i=1}^N\alpha_i}\leq 2\sqrt{\frac{4mn + \lambda^2N}{\lambda^2(N+\lambda^2)}}$.
\end{enumerate}
\end{lemma}

\begin{proof}
We can rearrange the indices so that $(\vx_i,y_i)$ are correct for $1\leq i\leq m$ and mislabeled for $m < i\leq N$. Without loss of generality, we can assume $y_i = 1$ for all $1\leq i\leq N$ by always replacing $y_i\vx_i$ by a new $\vx_i$. Now we have $x_{i,1}=1$ for $1\leq i\leq m$ and $x_{i,1}=-1$ for $m < i\leq N$. Note that $\frac {d-1}{\lambda^2}(\vx_i^\top \vx_i-1)$ is of distribution $\chi^2(d-1)$, a sum of $d-1$ iid sub-exponential $(4,4)$ random variables each with mean $1$. By the concentration results for sub-exponential random variables, we have
\begin{equation}
    \Pr\left[\left|\frac{d-1}{\lambda^2}(\vx_i^\top \vx_i-1)-(d-1)\right|\geq\varepsilon(d-1)\right]\leq 2\exp\left(-\frac{\varepsilon^2(d-1)}{8}\right), \forall 0\leq \varepsilon \leq 1.
\end{equation}
Similarly, when $1\leq i<j\leq N$, $\frac{d-1}{\lambda^2}(\vx_i^\top \vx_j-x_{i,1}x_{j,1})$ is a sum of $(d-1)$ iid sub-exponential $(2,2)$ random variables each with mean zero, so we have
\begin{equation}
    \Pr\left[\left|\frac{d-1}{\lambda^2}(\vx_i^\top \vx_j-x_{i,1}x_{j,1})\right|\geq \varepsilon(d-1)\right]\leq 2\exp\left(-\frac{\varepsilon^2(d-1)}{4}\right),\forall 0\leq \varepsilon \leq 1.
\end{equation}
%Define $\bm\alpha=(\alpha_1,\alpha_2,\cdots,\alpha_m,\beta_1,\beta_2,\cdots,\beta_n)^\top\in\bb R^{m+n}$. 
Define $A=(A_{ij})\in\bb R^{N\times N}$ such that $\forall 1\leq i\leq N,A_{ii}=1+\lambda^2,\forall 1\leq i<j\leq m,A_{ij}=A_{ji}=1,\forall m<i<j\leq N,
A_{ij}=A_{ji}=1,\forall 1\leq i\leq m<j\leq N,A_{ij}=A_{ji}=-1$. By the Union Bound, the above concentration results imply that $\forall 0\leq \varepsilon \leq 1$, with probability at least $1-2N^2\exp(-\frac{\varepsilon^2(d-1)}{8})$, every entry in $X^\top X$ differs from its corresponding entry in $A$ by at most $\varepsilon \lambda^2$.  As a consequence, with at least the probability, $\|X^\top X-A\|_\infty < \varepsilon\lambda^2N$, $\|X^\top X-A\|_1<\varepsilon \lambda^2N$ and $\|X^\top X-A\|\leq \|X^\top X-A\|_F<\varepsilon \lambda^2N$,  
where $\|\cdot\|_\infty,\|\cdot\|_1$ and $\|\cdot\|$ are the operator norm induced by $L_\infty$, the operator norm induced by $L_1$ and the spectral norm, respectively.
Let's choose \begin{equation}\varepsilon=\frac{(N+\lambda^2)}{2(2N-2+\lambda^2)N}\cdot\frac{\min\{2n + \lambda^2,m-n\}}{2m + \lambda^2}\in (0,1/N]\subseteq (0,1).
\end{equation}

Now, combining $\|X^\top X-A\| < \varepsilon \lambda^2N\leq \lambda^2$ and $\|A\|=N+\lambda^2$ gives $\|X^\top X\|\leq N + 2\lambda^2$. Therefore, $\sigma_{\max}(X)\leq \sqrt{N + 2\lambda^2}$. Note that the success probability $1-2N^2\exp(-\frac{\varepsilon^2(d-1)}{8})$ is at least $1-\delta$ by restraining $d\geq 2000\left(\frac{N(m+\lambda^2)}{\min\{2n+\lambda^2,m-n\}}\right)^2\ln\frac N\delta$. 


Note that the inverse of $A$ is $A^{-1}=(A^{-1}_{ij})\in\bb R^{N\times N}$ with $\forall 1\leq i\leq N,A^{-1}_{ii}=\frac{1}{\lambda^2}-\frac{1}{\lambda^2(N+\lambda^2)},\forall 1\leq i<j\leq m,A^{-1}_{ij}=A^{-1}_{ji}=-\frac{1}{\lambda^2(N+\lambda^2)},\forall m<i<j\leq N,A^{-1}_{ij}=A^{-1}_{ji}=-\frac{1}{\lambda^2(N+\lambda^2)},\forall 1\leq i\leq m<j\leq N,A^{-1}_{ij}=A^{-1}_{ji}=\frac{1}{\lambda^2(N+\lambda^2)}$. Therefore, $\|A^{-1}\|_\infty=\frac{2N-2+\lambda^2}{\lambda^2(N+\lambda^2)}$, which implies that $\min_{\vz\in\bb R^{N}:\|\vz\|_\infty=1}\|A\vz\|_\infty=\frac{\lambda^2(N+\lambda^2)}{2N-2+\lambda^2}$. Therefore, $\min_{\vz\in\bb R^{N}:\|\vz\|_\infty=1}\|X^\top X\vz\|_\infty\geq  \frac{\lambda^2(N+\lambda^2)}{2N-2+\lambda^2} - \|X^\top X-A\|_\infty > \frac{\lambda^2(N+\lambda^2)}{2N-2+\lambda^2}-\varepsilon\lambda^2N>0$ and thus $X^\top X$ is invertible and 
\begin{equation}\|(X^\top X)^{-1}\|_\infty< \left(\frac{\lambda^2(N+\lambda^2)}{2N-2+\lambda^2}-\varepsilon\lambda^2N\right)^{-1}.
\end{equation}
As a consequence, $X$ has full column rank. Define 
\begin{equation}
\rvc=\left(\underbrace{\frac{2n+\lambda^2}{\lambda^2(N+\lambda^2)},\cdots, \frac{2n+\lambda^2}{\lambda^2(N+\lambda^2)}}_{m},\underbrace{\frac{2m+\lambda^2}{\lambda^2(N+\lambda^2)},\cdots, \frac{2m+\lambda^2}{\lambda^2(N+\lambda^2)}}_{n}\right)^\top\in\bb R^{N}.
\end{equation}

% By standard concentration results, $\forall \varepsilon\in(0,1/2)$, with probability at least $1-C_1(m+n)^2\exp(-C_2\varepsilon^2d)$ for universal constants $C_1,C_2$, all of the following are true:
% \begin{enumerate}
% 	\item $\forall 1\leq i\leq N, |x_i^\top x_i-(1+\lambda^2)|< \varepsilon (1+\lambda^2)$;
% 	\item $\forall 1\leq i<j\leq m,|x_i^\top x_j-1|< \varepsilon (1+\lambda^2)$;
% 	\item $\forall m< i<j\leq N,|x_i^\top x_j-1|< \varepsilon (1+\lambda^2)$;
% 	\item $\forall 1\leq i\leq m < j\leq N,|x_i^\top x_j+1|<\varepsilon(1+\lambda^2)$.
% \end{enumerate} 
 


Suppose $\bm\alpha$ is the unique solution to the equation $X^\top X\bm\alpha=(\underbrace{1,\cdots,1}_{N})^\top$. We will prove that $\bm\alpha=(\alpha_1,\alpha_2,\cdots,\alpha_N)^\top$ satisfies statements 2, 3 and 4,
%Define $\hat w=X\bm\alpha$. We have $X^\top\hat w=(\underbrace{1,\cdots,1}_{N})^\top$. Therefore, $\forall i,\hat w^\top x_i=1,\hat w^\top y_i=1$. 
%Moreover, $\|\hat w\|_2^2=\hat w^\top \hat w=\bm\alpha^\top X^\top X\bm\alpha=\bm\alpha^\top (1,\cdots,1)^\top$. 
i.e., $\forall i,\alpha_i>0$ , $\min_{m< i\leq N}\alpha_i > \max_{1\leq j\leq m}\alpha_j$ and $\frac 12\sqrt{\frac{4mn + \lambda^2N}{\lambda^2(N+\lambda^2)}}\leq \sqrt{\sum_{i=1}^N\alpha_i}\leq 2\sqrt{\frac{4mn + \lambda^2N}{\lambda^2(N+\lambda^2)}}$. To show statements 2 and 3, we only need $\|\bm\alpha-\rvc\|_\infty< \min\left\{\frac{2n+\lambda^2}{\lambda^2(N+\lambda^2)},\frac{m-n}{\lambda^2(N+\lambda^2)}\right\}$. Note that $X^\top X\bm\alpha=(\underbrace{1,\cdots,1}_{N})^\top=A\rvc$, and thus $X^\top X(\rvc-\bm\alpha)=(X^\top X-A)\rvc$. Therefore, 
\begin{align}
\|\rvc-\bm\alpha\|_\infty\leq &\|(X^\top X)^{-1}\|_\infty\|(X^\top X-A)\|_\infty \|\rvc\|_\infty\nonumber \\
< &\left(\frac{\lambda^2(N+\lambda^2)}{2N-2+\lambda^2}-\varepsilon\lambda^2 N\right)^{-1}\varepsilon\lambda^2 N\cdot\frac{2m+\lambda^2}{\lambda^2(N+\lambda^2)}.\label{eq:1}
\end{align}
Recall that we chose  $\varepsilon=\frac{(N+\lambda^2)}{2(2N-2+\lambda^2)N}\cdot \frac{\min\{2n+\lambda^2,m-n\}}{2m+\lambda^2}$ which gives the desired $\|\bm\alpha-\rvc\|_\infty<\min\{\frac{2n+\lambda^2}{\lambda^2(N+\lambda^2)},\frac{m-n}{\lambda^2(N+\lambda^2)}\}$. 

Similarly, 
\begin{align}
\|\rvc-\bm\alpha\|_1\leq & \|(X^\top X)^{-1}\|_1\|(X^\top X-A)\|_1\|\rvc\|_1\nonumber \\
= &\|(X^\top X)^{-1}\|_\infty\|(X^\top X-A)\|_\infty\|\rvc\|_1\nonumber \\
< &\left(\frac{\lambda^2(m+n+\lambda^2)}{2m+2n-2+\lambda^2}-\varepsilon\lambda^2 N\right)^{-1}\varepsilon\lambda^2 N\cdot \|\rvc\|_1\nonumber \\
\leq & \frac 12\|\rvc\|_1.
\end{align}
Therefore, $\frac 14\cdot \frac{4mn+\lambda^2N}{\lambda^2(N+\lambda^2)}=\frac 14\|\rvc\|_1\leq \|\bm\alpha\|_1\leq 4\|\rvc\|_1=4\cdot \frac{4mn+\lambda^2N}{\lambda^2(N+\lambda^2)}$. Taking the squared root gives $\frac 12\sqrt{\frac{4mn+\lambda^2N}{\lambda^2(N+\lambda^2)}}\leq \sqrt{\sum_{i=1}^N\alpha_i}\leq 2\sqrt{\frac{4mn+\lambda^2N}{\lambda^2(N+\lambda^2)}}$.
\end{proof}
\begin{claim}
\label{claim:actual}
The $\bm\alpha$ defined in Lemma \ref{lm:mislabeleddual} is the actual optimal solution to the dual SVM program (\ref{eq:dual}). 
\end{claim}
\begin{proof}
Define $\hat \vw = X\bm\alpha$. We have $X^\top \hat \vw=X^\top X\bm\alpha = (1,1,\cdots,1)^\top$, so $\hat \vw$ is a feasible solution to the primal SVM program (\ref{eq:primal}) with objective value $\frac 12\|\hat \vw\|_2^2=\frac 12\hat \vw^\top \hat \vw=\frac 12\bm\alpha^\top X^\top X\bm\alpha=\frac 12\bm\alpha^\top (1,1,\cdots,1)^\top=\frac 12\sum_{i=1}^N\alpha_i$. Moreover, $\bm\alpha$ is a feasible solution to the dual (\ref{eq:dual})
% \begin{align*}
%     \text{Maximize }&\sum_{i=1}^N\alpha_i-\frac 12\sum_{i=1}^N\sum_{j=1}^N\alpha_i\alpha_jy_iy_jx_i^\top x_j,\\
%     \text{s.t. }&\forall 1\leq i\leq N,\alpha_i\geq 0,
% \end{align*}
with objective value $\sum_{i=1}^N\alpha_i-\frac 12\bm\alpha^\top X^\top X\bm\alpha=\sum_{i=1}^N\alpha_i-\frac 12\bm\alpha^\top (1,1,\cdots,1)^\top=\frac 12\sum_{i=1}^N\alpha_i$. Therefore, $\hat \vw$ is the global optimum of the primal and $\bm\alpha$ is the global optimum of the dual. %By complementary slackness, every $\alpha_i$ being positive means every training example being a support vector. Moreover, $\gamma^* = \left(\sum_{i=1}^N\alpha_i\right)^{-1/2} = \|\hat w\|_2^{-1}$ equals to the maximum normalized margin $\max_{\|w\|_2 = 1}\min_{1\leq i\leq N}y_iw^\top x_i$.
\end{proof}
\begin{remark}
\label{remark:margin}
Lemma \ref{lm:mislabeleddual}, together with Claim \ref{claim:margin} and Claim \ref{claim:actual}, implies that (under the same assumptions) with probability at least $1-\delta$ the optimal normalized margin for the training set is $\gamma^* = \left(\sum_{i=1}^N\alpha_i\right)^{-1/2}\leq 2\sqrt{\frac{\lambda^2(N+\lambda^2)}{4mn+\lambda^2N}}$, which can be arbitrarily close to zero as the size of the training set grows. This is in contrast to the case without mislabeling, where the optimal normalized margin is at least 1.
\end{remark}
\begin{proof}[Proof of Theorem \ref{thm:loss_separation_linear_re}]
% To combine Lemma \ref{lm:sgdratio_} and Lemma \ref{lm:mislabeleddual} to get Theorem \ref{thm:loss_separation_linear_re}, we first show that the $\bm\alpha$ defined in Lemma \ref{lm:mislabeleddual} is the actual optimal solution to the dual SVM program (\ref{eq:dual}). 

% % Consider the following hard-margin SVM program:
% % \begin{align*}
% %     \text{Minimize }&\frac 12\|\vw\|_2^2,\\
% %     \text{s.t. }&\forall 1\leq i\leq N, y_i\vw^\top \vx_i\geq 1.
% % \end{align*}
% Define $\hat \vw = X\bm\alpha$. We have $X^\top \hat \vw=X^\top X\bm\alpha = (1,1,\cdots,1)^\top$, so $\hat \vw$ is a feasible solution to the primal SVM program (\ref{eq:primal}) with objective value $\frac 12\|\hat \vw\|_2^2=\frac 12\hat \vw^\top \hat \vw=\frac 12\bm\alpha^\top X^\top X\bm\alpha=\frac 12\bm\alpha^\top (1,1,\cdots,1)^\top=\frac 12\sum_{i=1}^N\alpha_i$. Moreover, $\bm\alpha$ is a feasible solution to the dual (\ref{eq:dual})
% % \begin{align*}
% %     \text{Maximize }&\sum_{i=1}^N\alpha_i-\frac 12\sum_{i=1}^N\sum_{j=1}^N\alpha_i\alpha_jy_iy_jx_i^\top x_j,\\
% %     \text{s.t. }&\forall 1\leq i\leq N,\alpha_i\geq 0,
% % \end{align*}
% with objective value $\sum_{i=1}^N\alpha_i-\frac 12\bm\alpha^\top X^\top X\bm\alpha=\sum_{i=1}^N\alpha_i-\frac 12\bm\alpha^\top (1,1,\cdots,1)^\top=\frac 12\sum_{i=1}^N\alpha_i$. Therefore, $\hat \vw$ is the global optimum of the primal and $\bm\alpha$ is the global optimum of the dual. %By complementary slackness, every $\alpha_i$ being positive means every training example being a support vector. Moreover, $\gamma^* = \left(\sum_{i=1}^N\alpha_i\right)^{-1/2} = \|\hat w\|_2^{-1}$ equals to the maximum normalized margin $\max_{\|w\|_2 = 1}\min_{1\leq i\leq N}y_iw^\top x_i$.
%
Given the first claim in Lemma \ref{lm:mislabeleddual}, we know $X$ has full column rank and thus $(\vx_i)_{1\leq i\leq N}$ are linearly independent. Given the second claim in Lemma \ref{lm:mislabeleddual} and Claim \ref{claim:actual}, we know every dual value $\alpha_i$ is positive. In order to apply Lemma \ref{lm:sgdratio_} to prove Theorem \ref{thm:loss_separation_linear_re}, we only need to prove (\ref{eq:small_rate}) given the four properties claimed in Lemma \ref{lm:mislabeleddual}. The first and the fourth property in Lemma \ref{lm:mislabeleddual} imply $\sigma_{\max}(X)\leq \sqrt{N+2\lambda^2}$ and $\gamma^*\geq \frac 12\sqrt{\frac{\lambda^2(N+\lambda^2)}{4mn+\lambda^2N}}$. Therefore, 
\allowdisplaybreaks
\begin{align}
&\frac {\gamma^*}{2\beta\sigma^3_{\max}(X)(K+\sigma_{\max}(X)/\gamma^*)}\nonumber \\
\geq &\frac{\frac 12\sqrt{\frac{\lambda^2(N+\lambda^2)}{4mn + \lambda^2N}}}{2\beta(N+2\lambda^2)^{3/2}\left(K+2\sqrt{\frac{4mn+\lambda^2 N}{\lambda^2(N+\lambda^2)}}\cdot\sqrt{N+2\lambda^2}\right)}\nonumber \\
\geq & \frac 1{16\beta}\cdot\frac{\sqrt{\frac{\lambda^2}{4mn + \lambda^2N}}}{(N+\lambda^2)(K+4\sqrt{\frac{4mn+\lambda^2N}{\lambda^2}})}\nonumber \\
=&\frac 1{16\beta}\cdot \frac 1{(N+\lambda^2)(K\sqrt{4mn/\lambda^2 + N}+4(4mn/\lambda^2 + N))}\nonumber \\
\geq &\frac 1{256\beta}\cdot \left((N+\lambda^2)\left(K\sqrt{mn/\lambda^2+N}+mn/\lambda^2+N\right)\right)^{-1},
\end{align}
and
\allowdisplaybreaks
\begin{align}
&\frac 1{2K\beta\sigma_{\max}^2(X)}\nonumber \\
\geq &\frac 1{2\beta}\cdot \frac {1}{K(N+\lambda^2)}.
\end{align}
Therefore, the right-hand-side of (\ref{eq:small_rate}) is at least 
\begin{equation}
\frac 1{256\beta}\cdot \left((N+\lambda^2)\left(K\sqrt{mn/\lambda^2+N}+mn/\lambda^2+N\right)\right)^{-1},
\end{equation}
so restraining $\eta$ from exceeding this quantity satisfies (\ref{eq:small_rate}).
\end{proof}

==> 12_proof_deep.tex <==
\section{Theorem for Section \ref{subsec:loss_separation_deep}}

The following definition follows that given in \citep{wei2018margin}.
\begin{definition}[$a$-positive-homogeneous functions] We say $g:\bb R^{d_1}\rightarrow \bb R^{d_2}$ is $a$-positive-homogeneous for $a\in\bb R$ if $\forall c> 0,\forall w\in\bb R^{d_1}, g(cw)=c^ag(w)$.

\end{definition}
\begin{theorem}
\label{thm:loss_separation_deep}
Suppose we have $N$ training examples $(x_i,y_i)\in\bb R^{d_0}\times\{1,2,\cdots, K\}$ for $1\leq i\leq N$.  Suppose we train a classifier $f_w(x)\in\bb R^K$ with weights $w\in\bb R^d$.
% that takes $x\in\bb R^{d_0}$ and predicts its label $\hat y = \argmax_{1\leq i\leq K}f_w(x)[i]$. 
Suppose $f_w(x)$ is a continuously differentiable and $a$-positive-homogeneous function of $w$ for $a>0$, for example a deep network activated by $(\mathrm{ReLU}(\cdot))^{1.01}$. Let $w_\lambda\in\argmin\sum_{i=1}^N\ell(f_w(x_i),y_i)+\lambda\|w\|_2^2$, where the loss function $\ell(\cdot,\cdot)$ is the cross-entropy loss: $\ell(z,y)=-\ln(\frac{\exp(z[y])}{\sum_{1\leq j\leq K}\exp(z[j])})$. We define $\gamma(w)$ to be the margin of $w$ on the training set: $\gamma(w)=\min_{1\leq i\leq N, 1\leq j\leq K, j\neq y_i}(f_w(x_i)[y_i]-f_w(x_i)[j])$. Assume the training set is separable, i.e., there exists $w\in\bb R^d$ such that $\gamma(w)>0$. Suppose as $\lambda$ approaches $0^+$, $w_\lambda$ converges in direction to a max-margin solution $\hat w\in \argmin\{\|w\|_2:\gamma(w)\geq 1\}$. Assume $(\nabla_wf_w(x_i)[j]|_{w=\hat w})_{1\leq i\leq N,1\leq j\leq K}$ are linearly independent. Then $\hat w$ can be expressed as a linear combination of $(\nabla_wf_w(x_i)[j]|_{w=\hat w})_{1\leq i\leq N,1\leq j\leq K}$. Moreover, suppose $(\alpha_{i,j})_{1\leq i\leq N,1\leq j\leq K}\in\bb R^{N\times K}$ are the coefficients, i.e., $\hat w =\sum_{i=1}^N\sum_{j=1}^L\alpha_{i,j}\nabla_wf_w(x_i)[j]|_{w=\hat w}$, then
\begin{equation*}
    \lim\limits_{t\rightarrow +\infty}\frac{\ell(f_{w_t}(x_i),y_i)}{\sum_{j=1}^N\ell(f_{w_t}(x_j),y_j)}=\frac{\alpha_{i,y_i}}{\sum_{j=1}^N\alpha_{j,y_j}}.
\end{equation*}
\end{theorem}
% Suppose we have a sample of $m$ examples, $(x_1,y_1),(x_2,y_2),\cdots,(x_m,y_m)\in\bb R^d\times\{-1,1\}$ where $0<m<d$ (over-parameterized). Assume $x_1,x_2,\cdots,x_m$ are linearly independent. Assume the examples are linearly separable with max-margin solution $\hat w\neq \mathbf 0$ and corresponding dual solutions $\alpha_1,\alpha_2,\cdots,\alpha_m\in\bb R_{\geq 0}$ satisfying $\sum_{i=1}^m\alpha_iy_ix_i=\hat w$. Let $\ell(w;x,y)=\ell(yw^\top x)=\ln(1+\exp(-yw^\top x))$ be the Logistic loss. Suppose $w_\lambda$ is the global optimum of the following optimization problem:
% \begin{equation}
% \label{eq:opt1}
%     \text{Minimize }\sum\limits_{i=1}^m\ell(w;x_i,y_i)+\lambda\|w\|_2 \text{ over }w\in\bb R^d.
% \end{equation}
% Then, for any $1\leq j,k\leq m$ with $\alpha_k>0$, we have
% \begin{equation*}
%     \lim\limits_{\lambda\rightarrow 0^+}\frac{\ell(w_\lambda;x_j,y_j)}{\ell(w_\lambda;x_k,y_k)}=\frac{\alpha_j}{\alpha_k}.
% \end{equation*}

% \begin{proof}
% Since $w_\lambda$ is the global minimum of optimization problem (\ref{eq:opt1}), the gradient of the objective at $w_\lambda$ is zero:
% \begin{equation*}
%     \sum\limits_{i=1}^m\nabla_w\ell(w_\lambda;x_i,y_i)+2\lambda w_\lambda =0.
% \end{equation*}
% According to \cite{rosset2004margin} (Theorem 2.1), $w_\lambda$ direction converges to $\hat w$ as $\lambda$ approaches $0^+$, i.e., there exists $r_\lambda>0$ such that $w_\lambda=r_\lambda\hat w +o(r_\lambda)$ and $r_\lambda\rightarrow +\infty$ as $\lambda\rightarrow 0^+$. Therefore,
% \begin{equation*}
%     \sum\limits_{i=1}^m\nabla_w\ell(w_\lambda;x_i,y_i)+2\lambda r_\lambda \hat w + 2\lambda o(r_\lambda)=0
% \end{equation*}
% Substituting $\hat w = \sum_{i=1}^m\alpha_iy_ix_i$, $\nabla_w\ell(w_\lambda;x_i,y_i)=-(1+\exp(y_iw_\lambda ^\top x_i)^{-1}y_ix_i$ and dividing the equality by $2\lambda r_\lambda$, we get
% \begin{equation*}
%     \sum\limits_{i=1}^m(\alpha_i-\frac{1}{2\lambda r_\lambda}\cdot(1+\exp(y_iw_\lambda^\top x_i)^{-1})y_ix_i=o(1)
% \end{equation*}
% Therefore, noting that $x_i$ are linearly independent, we have $\forall 1\leq i\leq m,\lim\limits_{\lambda\rightarrow 0^+}\frac{1}{2\lambda r_\lambda}(1+\exp(y_iw_\lambda x_i)^{-1})=\alpha_i$, so
% \begin{equation*}
%     \lim\limits_{\lambda\rightarrow 0^+}\frac{(1+\exp(y_jw_\lambda^\top x_j))^{-1}}{(1+\exp(y_kw_\lambda^\top x_k))^{-1}}=\frac{\alpha_j}{\alpha_k}.
% \end{equation*}
% Finally, we complete the proof by noting that $y_jw_\lambda^\top x_j,y_kw_\lambda^\top x_k\rightarrow +\infty$ as $\lambda \rightarrow 0^+$ (see \cite{rosset2004margin}, Lemma 2.2), which implies $\lim_{\lambda\rightarrow 0^+}\frac{(1+\exp(y_jw_\lambda^\top x_j)^{-1}}{\ell(w_\lambda;x_j,y_j)}=1$ and $\lim_{\lambda\rightarrow 0^+}\frac{(1+\exp(y_kw_\lambda^\top x_k)^{-1}}{\ell(w_\lambda;x_k,y_k)}=1$.
% \end{proof}

% The following lemma can be proved by following the analysis of \cite{soudry2017implicit, nacson2018stochastic}.


% \begin{lemma}
% \label{lm:weakregdeep}
% Suppose we have a sample of $m$ examples, $(x_1,y_1),(x_2,y_2),\cdots,(x_m,y_m)\in\bb R^{d_1}\times\{-1,1\}$. Let $\ell(w;x,y)=\ell(yf_w(x))=\ln(1+\exp(-yf_w(x)))$ be the Logistic loss associated with neural network $f_w(x)\in\bb R$ parameterized by $w\in\bb R^d$. Suppose $d>m$ (over-parameterized). Suppose the neural network is continuously differentiable and positive-homogeneous of order $\sigma>0$ (for example, a neural network with activation function $\mathrm{activation}(z)=(ReLU(z))^{1.01}$). Suppose $w_\lambda$ is one of the global optimizers of the following optimization problem:
% \begin{equation}
% \label{eq:opt2}
%     \text{Minimize }\sum\limits_{i=1}^m\ell(w;x_i,y_i)+\lambda\|w\|_2\text{ over }w\in\bb R^d,
% \end{equation}
% and suppose $w_\lambda$ direction converges to $\hat w$, i.e., there exists $r_\lambda >0$ such that $w_\lambda = r_\lambda\hat w+o(r_\lambda)$ with $r_\lambda\rightarrow +\infty$ as $\lambda \rightarrow 0^+$. Suppose $\hat w$ fits the data perfectly: $\forall 1\leq i\leq m,y_if_{\hat w}(x_i)>0$. Assume $(\nabla_w\ell(\hat w;x_i,y_i))_{1\leq i\leq m}$ are linearly independent. Then there exist $\alpha_1,\alpha_2,\cdots,\alpha_m\in\bb R_{\geq 0}$ satisfying $\sum_{i=1}^m\alpha_iy_i\nabla_wf_{\hat w}(x_i)=\hat w$ and for all $1\leq j,k\leq m$ with $\alpha_k>0$, we have
% \begin{equation*}
%     \lim\limits_{\lambda\rightarrow 0^+}\frac{\ell(w_\lambda;x_j,y_j)}{\ell(w_\lambda;x_k,y_k)}=\frac{\alpha_j}{\alpha_k}.
% \end{equation*}
% \end{lemma}
\begin{proof}
Since $w_\lambda$ optimizes $\sum_{i=1}^N\ell(f_w(x_i),y_i)+\lambda\|w\|_2^2$, the gradient at $w_\lambda$ is zero:
\begin{equation*}
    \sum\limits_{i=1}^N\nabla_w\ell(f_w(x_i),y_i)|_{w=w_\lambda}+2\lambda w_\lambda = 0.
\end{equation*}
Define $\beta_{i,y_i}(w)=\frac{\sum_{1\leq k\leq K,k\neq y_i}\exp(f_{w}(x_i)[k])}{\sum_{1\leq k\leq K}\exp(f_{w}(x_i)[k])}$ and $\beta_{i,j}(w)=-\frac{\exp(f_{w}(x_i)[j])}{\sum_{1\leq k\leq K}\exp(f_{w}(x_i)[k])}$ for $1\leq i\leq N,1\leq j\leq K,j\neq y_i$.
Note that $\nabla_w\ell(f_w(x_i),y_i)=-\sum_{j=1}^K\beta_{i,j}(w)\nabla_wf_w(x_i)[j]$, we have
\begin{equation*}
    -\sum\limits_{i=1}^N\sum\limits_{j=1}^K \beta_{i,j}(w_\lambda)\nabla_wf_{w}(x_i)[j]|_{w=w_\lambda}+2\lambda w_\lambda = 0.
\end{equation*}
Note that $\min_{\|w\|_2=R}\sum_{i=1}^N\ell(f_w(x_i),y_i)\rightarrow 0$ as $R\rightarrow +\infty$, so $\|w_\lambda\|_2\rightarrow +\infty$ as $\lambda\rightarrow 0^+$. Therefore, we can assume $w_\lambda = r_\lambda \hat w + o(r_\lambda)$ for $r_\lambda\rightarrow +\infty$ as $\lambda\rightarrow 0^+$. Note that $\nabla_wf_w(x)$ is $(a-1)$-positive-homogeneous, we know
\begin{equation*}
    -r_\lambda ^{a - 1}\sum\limits_{i=1}^N\sum\limits_{j=1}^K \beta_{i,j}(w_\lambda)\nabla_wf_w(x_i)[j]|_{w=\frac{w_\lambda}{r_\lambda}}+2\lambda w_\lambda = 0.
\end{equation*}
Dividing the equality by $2\lambda r_\lambda$ and noting that $w_\lambda = r_\lambda \hat w + o(r_\lambda)$, we have:
\begin{equation*}
    -\frac {r_\lambda^{a - 2}}{2\lambda}\sum\limits_{i=1}^N\sum\limits_{j=1}^K\beta_{i,j}(w_\lambda)\nabla_wf_{w}(x_i)[j]|_{w=\frac{w_\lambda}{r_\lambda}} + \hat w = o(1).
\end{equation*}
Note that $f$ is continuously-differentiable, so we know $\lim\limits_{\lambda\rightarrow 0^+}\nabla_wf_{w}(x_i)[j]|_{w=\frac{w_\lambda}{r_\lambda}}=\nabla_wf_{w}(x_i)[j]|_{w=\hat w}$, which are linearly independent for $1\leq i\leq N,1\leq j\leq K$. Therefore, $\max_{1\leq i \leq N,1\leq j\leq K}\left|-\frac{r_\lambda^{a - 2}}{2\lambda}\beta_{ij}(w_\lambda)\right|$ is bounded uniformly for $\lambda$ sufficiently close to $0^+$. Consequently,
\begin{equation*}
    -\frac {r_\lambda^{a - 2}}{2\lambda}\sum\limits_{i=1}^N\sum\limits_{j=1}^K\beta_{i,j}(w_\lambda)\nabla_wf_{w}(x_i)[j]|_{w=\hat w} + \hat w = o(1).
\end{equation*}
Therefore, $\forall 1\leq i\leq N,1\leq j\leq K$ we have $\lim\limits_{\lambda\rightarrow 0^+}\frac{r_\lambda^{a - 2}}{2\lambda}\beta_{i,j}(w_\lambda)=\alpha_{i,j}$, where $\sum\limits_{i=1}^N\sum\limits_{j=1}^K\alpha_{i,j}\nabla_wf_{w}(x_i)[j]|_{w=\hat w}=\hat w$. 

Note that $\forall 1\leq i\leq N,\forall w\in\bb R^d,\sum_{j=1}^K\beta_{i,j}(w)=0$, and $\beta_{i,y_i}>0>\beta_{i,j}$ for $j\neq y_i$. Therefore, $\forall 1\leq i\leq N,\sum_{j=1}^K\alpha_{i,j}=0$ and $\alpha_{i,y_i}\geq 0\geq \alpha_{i,j}$ for $j\neq y_i$. Therefore, $\sum_{i=1}^N\alpha_{i,y_i}>0$, because otherwise we would get $\alpha_{i,j}=0$ for all $1\leq i\leq N,1\leq j\leq K$, a contradiction with $\hat w\neq 0$.

Now we have $\forall 1\leq i\leq N$,
\begin{equation}
\label{eq:beta_ratio}
    \lim\limits_{\lambda \rightarrow 0^+}\frac{\beta_{i,y_i}(w_\lambda)}{\sum_{j=1}^N\beta_{j,y_j}(w_\lambda)}=\frac{\alpha_{i,y_i}}{\sum_{j=1}^N\alpha_{j,y_j}}.
\end{equation}
Finally, note that
\begin{align*}
\lim_{\lambda\rightarrow 0^+}\frac{\ell(f_{w_\lambda}(x_i),y_i)}{\beta_{i,y_i}(w_\lambda)}=&\lim_{\lambda\rightarrow 0^+}\ell(f_{w_\lambda}(x_i),y_i)\cdot \frac{\sum_{1\leq k\leq K}\exp(f_{w_\lambda}(x_i)[k])}{\sum_{1\leq k\leq K,k\neq y_i}\exp(f_{w_\lambda}(x_i)[k])}\\
=&\lim_{\lambda\rightarrow 0^+}\ell(f_{w_\lambda}(x_i),y_i)\cdot\frac{\exp(f_{w_\lambda}(x_i)[y_i])}{\sum_{1\leq k\leq K,k\neq y_i}\exp(f_{w_\lambda}(x_i)[k])}\cdot\frac{\sum\limits_{1\leq k\leq K}\exp(f_{w_\lambda}(x_i)[k])}{\exp(f_{w_\lambda}(x_i)[y_i])}\\
=&\lim_{\lambda\rightarrow 0^+}\ell(f_{w_\lambda}(x_i),y_i)\cdot\frac{\exp(f_{w_\lambda}(x_i)[y_i])}{\sum_{1\leq k\leq K,k\neq y_i}\exp(f_{w_\lambda}(x_i)[k])}\\
=&\lim_{\lambda\rightarrow 0^+}\ln\left(1+\frac{\sum_{1\leq k\leq K,k\neq y_i}\exp(f_{w_\lambda}(x_i)[k])}{\exp(f_{w_\lambda}(x_i)[y_i])}\right)\cdot \frac{\exp(f_{w_\lambda}(x_i)[y_i])}{\sum_{1\leq k\leq K,k\neq y_i}\exp(f_{w_\lambda}(x_i)[k])}\\
=&\lim\limits_{\lambda\rightarrow 0^+}\frac{\sum_{1\leq k\leq K,k\neq y_i}\exp(f_{w_\lambda}(x_i)[k])}{\exp(f_{w_\lambda}(x_i)[y_i])}\cdot \frac{\exp(f_{w_\lambda}(x_i)[y_i])}{\sum_{1\leq k\leq K,k\neq y_i}\exp(f_{w_\lambda}(x_i)[k])}\\
=&1,
\end{align*}
which further implies $\lim\limits_{\lambda\rightarrow 0^+}\frac{\sum_{j=1}^N\ell(f_{w_\lambda}(x_j),y_j)}{\sum_{j=1}^N\beta_{j,y_j}(w_\lambda)}=1$. Combining with (\ref{eq:beta_ratio}), we get
the desired equality.
\end{proof}

==> 6_theory.tex <==
\section{A Theoretical Viewpoint}
\label{sec:theory}
In this section, we give a theoretical justification for using the losses to distinguish the clean examples and the mislabeld ones, in a simplified setting with binary linear classifiers. We show that the losses contain more information than the binary error: even if the model overfits to the wrong label of a mislabeled example, we may still identify the mislabeling by observing a loss that is significantly larger than the average loss. 


We note that it's challenging to rigorously characterize the statistical properties of the SGD iterates in deep learning, and so is to extend our results on the loss distribution to deep models and theoretically explain all of our techniques. (Please see~\cite{mandt2017stochastic, dinh2017sharp} and the references therein for some recent studies.) We consider our main contribution to be the empirical success, and the mathematical reasoning here only serves as a complement to the experiments. 


%we give a theoretical explanation for the separation of the loss of mislabeled examples from the loss of correct examples during training.
%, and how generalization can be significantly improved by making use of this separation. 


% For the ease of exposition, here we consider binary classification. 
% (The theory can extended to multi-label cases without much modification, see Section~\ref{?} in supplementary materials. \lh{Not sure if we can extend to multi-class without weak regularization, because \citep{nacson2018stochastic} didn't have the corresponding result for SGD. \citep{soudry2017implicit} did have the result for GD, though. }
Let $(\vx_1, y_1),\cdots,(\vx_N, y_N)$ be a set of training examples  sampled iid from a distribution over $\bb R^d\times\{\pm 1\}$.
Let $f_\vw(\vx) = \vw^\top \vx$ be a linear classifier with parameter $\vw\in\bb R^d$, which predicts label $\hat y = 1$ if $f_\vw(\vx)\geq 0$ and $\hat y = -1$ otherwise. Because deep neural nets are often over-parametrized, we also assume here the number of data points is smaller than the number of parameters, that is, $N < d$. In this case, when $\vx_1, \vx_2,\cdots, \vx_N$ are linearly independent, for any  labels (with or without mislabeling), there always exists a linear classifier with zero training error.

We analyze SGD on the empirical logistic loss.
% without $\ell_2$ regularization for simplicity (Section~\ref{} extends it to objective with $\ell_2$ regularization.\lh{Here the extension means the weak regularization analysis?}) 
Concretely, the training objective is 
\begin{equation}
\textup{Minimize}_\vw \sum\limits_{i=1}^N \ell(\vw; \vx_i,y_i),\label{eqn:obj}
\end{equation}
where $\ell(\vw; \vx_i,y_i)=\ln(1+\exp(-y_i\cdot \vw^\top \vx_i))$. 

% Recently, \citep{soudry2017implicit, nacson2018stochastic} proved that with sufficiently small constant learning rate, SGD iterates converge in direction to the max-margin (hard-margin SVM) solution, assuming the training set is linearly separable. Building upon tools from these works, we first show that in the run of SGD, the ratio of the logistic losses of any two training examples $(\vx_i,y_i),(\vx_j,y_j)$ converges to the ratio of the corresponding values $\alpha_i,\alpha_j$ in the optimal solution to the following dual (hard-margin)  SVM program: %Let $\alpha_1,\dots, \alpha_N$ be the optimal values of the dual variables of  the examples; that is, the optimal solution to the dual SVM program 
% \begin{equation}
% \label{eq:dual}
% \begin{split}
% \textup{Maximize }&\sum_{i=1}^N\alpha_i-\frac 12\sum_{i=1}^N\sum_{j=1}^N\alpha_i\alpha_jy_iy_j\vx_i^\top \vx_j\\
% \textup{s.t. } & \alpha_1,\cdots,\alpha_N\geq 0.
% \end{split}
% \end{equation}
% Specifically, let $\vw_t$ be the $t$-th iterate of SGD with mini-batch\footnote{Technically, we require all mini-batches to have the same size and each example to be selected in exactly one mini-batch in every epoch.} and constant learning rate $\eta$ on the objective (\ref{eqn:obj}) from any initialization $\vw_0$. We show the following lemma:

% \begin{lemma}
% \label{lm:sgdratio}
% In the setting above, for almost all training sets with respect to the Lebesgue measure, for sufficiently small learning rate $\eta$, the ratio of losses of any two examples $(\vx_i,y_i)$ and $(\vx_j,y_j)$ with $\alpha_j>0$ satisfies
% \begin{equation}
% \lim\limits_{t\rightarrow \infty}\frac{\ell(\vw_t;\vx_i,y_i)}{\ell(\vw_t;\vx_j,y_j)}=\frac{\alpha_i}{\alpha_j}.
% \end{equation}
% %\lh{Need linear independence. Need every $\alpha_i>0$.}
% \end{lemma}

% With this connection in hand, it suffices to understand the optimal dual values $\alpha_1,\dots, \alpha_N$ for clean and mislabeled examples. We will argue that mislabeled examples tend to have higher optimal dual values than clean examples: the dual variables capture how much an example influences the separating hyperplane --- recall that by duality, the SVM solution can be written as $\hat \vw = \alpha_1y_1\vx_1+\dots + \alpha_Ny_N\vx_N$. Intuitively, mislabeled examples will contribute more to the supporting hyperplane since they tend to cause more element of surprises and influence the decision boundary more than the clean examples. 

% The precise reflection of the intuition above generally depends on the particular data distributions and the distribution of the mislabeled examples. 

We consider the following simplified setting of the data distribution,
under which we can show sharp separation between the clean and mislabeled examples by losses. 

%We will first consider linear binary classification. 
%\citet{nacson2018stochastic} showed SGD over the logistic loss converges in direction to the max-margin solution. In the case where the training set allows a large normalized margin, SGD finds the max-margin solution and thus provably exhibits good generalization performance even when the classifier is over-parameterized (the dimension is much higher than the number of training examples). However, a small portion of mislabeled examples in the training set could easily cause over-fitting: the training error could still reach down to zero, and SGD still finds the max-margin solution, but the normalized margin would be significantly reduced.
%% , and in this case the max-margin solution found by SGD no longer generalizes and could perform nearly as bad as random guess on test data even when the training error is still zero due to over-parameterization. 
%We show that for certain cases like this, after sufficiently long training using SGD over the logistic loss, mislabeled examples always have larger loss than correct examples (Theorem \ref{thm:loss_separation_linear}), despite that the loss of every training example eventually converges to zero. We can then hope to remove the mislabeled examples from the training set by looking at the loss and find the (desirable) max-margin solution for the correct examples.

%This implicit bias of SGD towards fitting correct examples faster than mislabeled ones has the following structure. First, the ratio between the loss of any two examples in the training set converges to the ratio of their corresponding dual variables in the hard-margin SVM solution. Second, mislabeled examples correspond to larger dual variables compared to correct examples. 
%The second part is not surprising, as when the training set is not linearly separable, all the training examples that are not classified correctly have dual variables reaching the upper limit in soft-margin SVM. 

%\subsection{Linear Binary Classification}
%Imagine we have a set of training examples $(x_1,y_1),\cdots,(x_N,y_N)$ sampled iid from a distribution $\mc D$ over $\bb R^d\times\{\pm 1\}$. Suppose we train a linear classifier $f_w(x)=w^\top x$ with parameter $w\in\bb R^d$ that predicts for $x\in\bb R^d$ a label $\hat y = 1$ if $f_w(x)\geq 0$ and $\hat y = -1$ if $f_w(x)<0$. We assume our model is over-parameterized, i.e., $m < d$. In this case, it's typical that $x_1,x_2,\cdots,x_N$ are linearly independent, and as a consequence there exists a parameter $w\in\bb R^d$ that makes the correct prediction for every training example: $\forall 1\leq i\leq N,y_if_w(x_i)>0$, no matter what the labels $(y_i)_{1\leq i \leq N}$ are.

%%Note that $f_w(x)$ is a homogeneous function of $w$, so it's without loss of generality to restrain $w$ to have $L_2$ norm at most 1. In this case, the empirical Rademacher complexity of $f_w(x)$ has an upper bound $\sqrt{\frac{L}{m}}$, where $L=\frac{\sum_{i=1}^m\|x_i\|_2^2}{m}$. Therefore, 
%According to the margin theory, with high probability, the generalization error for the learned parameter $w$ is at most $O\left(\frac{\|w\|_2}{\gamma(w)}\sqrt{\frac{L}{N}}\right)$, where $\gamma(w)$ is the margin associated with $w$, i.e., $\gamma(w) = \min_{1\leq i \leq N}y_if_w(x_i)$, and $L$ is the average squared norm of the training examples: $L=\frac{\sum_{i=1}^N\|x_i\|_2^2}{N}$. This tells us that if we could find a solution with a large normalized margin, i.e., $\frac{\gamma(w)}{\|w\|_2}$ is at least comparable with $\sqrt{L}$, then we get better and better generalization as we increase $N$, the size of the training set, even if the dimension $d$ is far larger. This is why we want the max-margin solution $\hat w = \argmin\{\|w\|_2:\gamma(w)\geq 1\}$.

Let $x_{i,j}$ be the $j$-th coordinate of the example $\vx_i$. We assume that the first coordinate of each example $x_{i,1}$ always coincides with the correct label, that is, $x_{i,1} = \bar{y}_i$, where we use $\bar{y}_i\in \{-1,+1\}$ to denote the correct label. The rest of the coordinates of all the examples are i.i.d generated from $\mc N\left(0,\frac {\lambda^2}{d-1}\right)$ for some constant $\lambda$.\footnote{$\lambda$ can also grow with the dimension. See the restatement of Theorem~\ref{thm:loss_separation_linear} in Appendix \ref{sec:proof_loss_separation_linear} for details. } Note that each example has expected squared norm $1+\lambda^2$, and the classifier $\vw^* = (1,0,\dots,0)$ classifies all the examples with margin 1 when all the labels are correct. Now we choose $n <N/2$ random examples among these $N$ examples, and flip the label $\bar{y}_i$ for them to get the wrong label $y_i = -\bar{y}_i$, and for the rest of the examples we set $y_i =\bar{y}_i$. This synthetic dataset has $n<N/2$ mislabeled examples, but since we assumed $d > N$, the dataset can still be overfit to training error zero.
%\footnote{The noisy training set is linearly separable due to over-parametrization, but the optimal normalized margin can be arbitrarily close to zero (see Remark \ref{remark:margin} in Appendix \ref{sec:proof_loss_separation_linear}).} 
We show that by comparing the losses we can identify the correct and mislabeled examples:

%
%\tnote{what is $L$? do we need mention $\gamma, L$ for the purpose of this section?}
%
%\lh{I mentioned that just to argue the distribution allows good generalization if there is no mislabeled examples, and the margin can decrease dramatically with mislabeled examples.}
%
%\tnote{what's the conditions for $\lambda$? I thougth we need $\lambda$ to be somewhat large?}
%
%\lh{We need $\lambda$ not to be too large relatively to the size of training set and the dimension $d$.}

%
% $x_i=(x_{i,1},x_{i,2}\cdots,x_{i,d})$ satisfies that $x_{i,1}=y_i$ and $x_{i,j}$ is independently from $\mc N\left(0,\frac {\lambda^2}{d-1}\right)$ for $2\leq j\leq d$ for some constant $\lambda > 0$. For large enough $d$, $L$ concentrates around $1 + \lambda^2$, while $\gamma^*$ is at least 1. Up to scaling and rotation, we can produce other data distributions with this large margin property.  \citet{nacson2018stochastic} showed that SGD over the logistic loss converges in direction to the max-margin solution $\hat w$, and thus SGD has provably good generalization in this case. However, if we flip the labels of a small random portion of the training set, the maximum possible normalized margin could be arbitrarily close to zero (Remark A.1 in Supplementary). 
% Part of the reason is that \emph{although it's desirable to take the max-margin solution among all solutions that fit all the training examples, it's not desirable to take a solution that fits all the training examples in the first place, especially when there are noisy examples with wrong labels.} 
%We prove the following theorem showing separation of the loss of mislabeled and correct training examples so that in principle we can hope to delete the mislabeled examples from the training set to achieve as good margin as in the case of no mislabeled examples.
\begin{theorem}
\label{thm:loss_separation_linear}
On the synthetic datasets discussed above, for sufficiently small $\eta$, sufficiently large $d$, with high probability over the randomness of the training set, there exists some time $T>0$ such that for all $t>T$, all the mislabeled examples (in $\gB$) have bigger loss than the clean ones (in $\gG$):
\begin{equation}
    \min_{i: {(\vx_i,y_i) \in \gB}}%\text{ is mislabeled}}}
    \ell(\vw_t; \vx_i,y_i)>\max_{j: {(\vx_j,y_j)  \in \gG}} %\text{is clean}}}
    \ell(\vw_t; \vx_j,y_j).
\end{equation}
\end{theorem}

%The proof of Theorem is deferred to Section~\ref{?}. Finally, we remark that Lemma~\ref{??} does not limit to linear classification: for non-linear models, the ratio of the losses do converge to some fixed value only depends on the data.    by analyzing the global optimum of the weakly regularized problem (a similar setting as in \citep{rosset2004margin, wei2018margin}), we show for multi-class deep-network classifiers, the ratio of the cross entropy loss of any two training examples converges as the regularization strength vanishes to zero under certain assumptions (Theorem B.1 in Supplementary), revealing a bias towards fitting \emph{some} training examples better than \emph{others}.

% \tnote{need to decide on how to phrase the multi-layer results. what does the ratio of the loss converges to? the ratio converges as $t$ goes to infinity or as $\lambda$ goes to zero? (Let's say one can assume direction converges of the iterates)}

% \lh{In the linear multi-class case, the convergence is to the multi-class SVM dual. For deep classifiers, I don't think we can interpret the limit as some kind of dual variables, but it's some value determined only by the training set, the loss function and the max-margin solution (independent of $\lambda$). Convergence is for $\lambda\rightarrow 0^+$.}
% \subsection{Extensions to Multi-Class Deep-Net Classifiers via Weak Regularization Analysis}
% \label{subsec:loss_separation_deep}
% The phenomenon that optimizing the logistic loss yields the max-margin solution was shown not limited to linear binary classification. Recently, \citet{wei2018margin}, building on the work of \citet{rosset2004margin}, showed for non-linear positive-homogeneous $K$-class classifiers $f_w(x)\in\bb R^K$ such as deep ReLU networks 
% % where $\hat y_i:=\argmax_{1\leq j\leq K}f_w(x)[j]$ is the predicted label 
% that if we add a weak $L_2$-regularizer term $\lambda\|w\|_2^2$ to the optimization problem of the cross entropy loss, the normalized margin of the global optimum converges to the maximum possible normalized margin as the regularization strength $\lambda$ vanishes to zero. If we further assume that the global optimum converges in direction to a max-margin solution 
% %$\hat w\in\argmin\{\|w\|_2:\min_{1\leq i\leq N,1\leq j\leq K,j\neq y_i}f_w(x_i)[y_i]-f_w(x_i)[j]\geq 1\}$
% and certain other assumptions, we can prove 
% %the following theorem showing 
% that for multi-class deep-nets, the ratio between the loss of any two training examples also converges (Theorem \ref{thm:loss_separation_deep}).
% \begin{theorem}
% \label{thm:multi_class_deep}
% Suppose we have $N$ training examples $(x_i,y_i)\in\bb R^{d_0}\times\{1,2,\cdots, K\}$ for $1\leq i\leq N$. Suppose we train a classifier $f_w:\bb R^{d_0}\rightarrow \bb R^K$ with weights $w\in\bb R^d$.
% % that takes $x\in\bb R^{d_0}$ and predicts its label $\hat y = \argmax_{1\leq i\leq K}f_w(x)[i]$.
% Suppose $f_w(x)$ is a continuously differentiable and $a$-positive-homogeneous (see Definition B.1 in Supplementary) function of $w$ for $a>0$, for example a deep network activated by $(\mathrm{ReLU}(\cdot))^{1.01}$. Let $w_\lambda\in\argmin\sum_{i=1}^N\ell(f_w(x_i),y_i)+\lambda\|w\|_2^2$ be a global optimum of the weakly regularized problem, where the loss function $\ell(\cdot,\cdot)$ is the cross-entropy loss: $\ell(z,y)=-\ln(\frac{\exp(z[y])}{\sum_{1\leq j\leq K}\exp(z[j])})$.  Suppose as $\lambda$ approaches $0^+$, $w_\lambda$ converges in direction to a max-margin solution $\hat w$. Assume $(\nabla_wf_w(x_i)[j]|_{w=\hat w})_{1\leq i\leq N,1\leq j\leq K}$ are linearly independent. Then $\hat w$ can be expressed as a linear combination of $(\nabla_wf_w(x_i)[j]|_{w=\hat w})_{1\leq i\leq N,1\leq j\leq K}$. Moreover, suppose $(\alpha_{i,j})_{1\leq i\leq N,1\leq j\leq K}\in\bb R^{N\times K}$ are the coefficients, i.e., $\hat w =\sum_{i=1}^N\sum_{j=1}^K\alpha_{i,j}\nabla_wf_w(x_i)[j]|_{w=\hat w}$, then $\forall 1\leq i\leq N$,
% \begin{equation*}
%     \lim\limits_{t\rightarrow +\infty}\frac{\ell(f_{w_t}(x_i),y_i)}{\sum_{j=1}^N\ell(f_{w_t}(x_j),y_j)}=\frac{\alpha_{i,y_i}}{\sum_{j=1}^N\alpha_{j,y_j}}.
% \end{equation*}
% \end{theorem}

==> garbage.tex <==
% Simple case, binary classification problem, $\rvx \sim \mc{N}(0, I)$ (or have the same norm, just so the gradient of parameters translates from the gradient over the logits), and $y \in [0, 1]$, there are two datasets $\mc{G}$ and $\mc{B}$, where $\mc{B}$ has higher variance (e.g. the labels in $\mc{B}$ are all either 1 or 0 w.p 0.5 independent of inputs). Assuming the network has infinite capacity, it can either fit all $\mc{G}$ or $\mc{G} \cup \mc{B}$. The gradient and hessian over label $y_n$ with logits $\hat{y_n}$ are:
% $$
% \nabla_{\hat{y}_n} = \frac{y_n}{\hat{y_n}} - \frac{1 - y_n}{1 - \hat{y_n}}
% $$
% and
% $$
% \nabla^2_{\hat{y}_n} = \frac{y_n}{\hat{y_n}^2} + \frac{1 - y_n}{(1 - \hat{y_n})^2}
% $$
% \begin{itemize}
% \item In the case where $\mc{G}$ are all fitted but the network produces $0.5$ for $\mc{B}$, $\nabla = 0$, and $\nabla^2 = \nabla^2_{\mc{G}} + |\mc{B}|0.25$
% \item In the case where $\mc{B}$ are also fitted, $\nabla = 0$, and $\nabla^2 = \nabla^2_{\mc{G}} + \nabla^2_{\mc{B}}$, which is larger than the previous case.
% \end{itemize}

% \js{find an example that explains the large lr thing}

% We can utilize this implicit regularization effect to remove examples that might harm generalization, leading to \textsc{Noise Classifier}, a simple algorithm highly robust to mislabeled / noisy examples:

% \begin{enumerate}
%     \item Train all examples with large learning rates for $E$ epochs.
%     \item Determine a threshold $T$ to classify ``good'' examples and ``bad'' ones.
%     \item Prune examples whose average loss of the past $h$ epochs exceeds $T$ from the dataset.
%     \item Continue training the remaining examples from epoch $E+1$.
% \end{enumerate}

% \textsc{Noise Classifier} introduces three hyperparameters: $E$ determines the amount of training that separate clean examples from noisy ones; $p$ determines $T_p$ that specifies the trade-off between less noisy examples and more clean examples; $h$ determines the window of averaged loss statistics to reduce variance from data augmentation. We do not explicitly estimate the portion of noise in the dataset, nor do we assume any specific noise model. In fact, the threshold $T_p$ could be used to accurately predict the portion of uniform noise in the dataset, and works quite well even on other types of label noise; we will demonstrate this in Section~\ref{sec:experiments}.

% Our algorithm can be easily adapted from existing supervised training procedures. \textsc{Noise Classifier} merely requires $\mathcal{O}(Nh)$ more memory to store the loss values, as well as simulating $p_n(\ell)$ at epoch $E$ to compute $T_p$. Compared to the cost of training these neural networks, the additional computational overhead is almost negligible. We discuss more implementation details in \js{appendix}.

% Denote $\ell_i(\theta) = \log p_\theta(\rvy_i|\rvx_i)$ is the log-likelihood of a particular example. The weighted objective is $\mc{L}(w; \theta) = \sum_{i \in \mc{I}} w_i \ell_i(\theta) / \sum_{i \in \mc{I}} w_i$, the original objective is $\mc{L}(\vone; \theta)$. 

% Given a (clean) validation set not accessed by our algorithm during training $\valid = (\rvx_j, \rvy_j)_{j \in \mc{V}}$, our goal is to find $\theta$ that minimizes the validation loss $\mc{L}_{val}(\vone; \theta) = \sum_{j \in \mc{V}} \ell_j(\theta) / |\mc{V}|$.

% \textbf{Assumption 1 (informal)}: the training error on clean set is closest to validation error (e.g. measure distance under FIM). Or, generalization gap is smallest if we use $\mc{L}(\rvw_{\mc{C}}; \theta)$ where $\rvw_{\mc{S}}$ is ``indicator function'' (so it ignores mislabeled examples).

% \textbf{Assumption 2 (informal)}: the training error on mislabeled set is orthogonal to validation error (not sure if it is required, exists to address class-dependent mislabeling)

% Our algorithm does not have access to $\mc{M}$ and $\mc{C}$ (otherwise, a trivial solution is to train with $\mc{L}(\rvw_{\mc{C}}; \theta)$, i.e. clean labels only). Hence to minimize the generalization gap, we need to identify $\mc{M}$ and $\mc{C}$.

% (Paraphrasing Yann's argument, very informal) at large learning rate (large noise for SGD), the magnitude/direction of $\nabla_\theta \mc{L}(\rvw_{\mc{C}}; \theta)$ dominates training; however, as training continues into small learning rate regimes, the magnitude of $\nabla_\theta \mc{L}(\rvw_{\mc{M}}; \theta)$ dominates training (since $\mc{L}(\rvw_{\mc{C}}; \theta)$ is close to zero).


% \subsection{Description}
% \begin{itemize}
% \item We observe that the loss distribution for noise does not change much at the beginning of training (with large lrs)
% \item In fact, the loss distribution for noise can be simulated by this:
% $$\textrm{loss} = \log \textrm{softmax}(x) \quad x \sim N(0, I)$$
% \item This only depends on the number of labels in the task, and does not depend on the \% of corrupted labels.
% \item The variance of 1 could be related to how ResNets are parametrized with batch norm.
% \item One could also obtain the loss distribution by assuming the last layer batch norm produces $N(0, I)$ noise.
% \item For our threshold, we take the $p$-th percentile for the loss distribution for noise. This ensures that our noise classifier has around $(1 -  p\%)$ recall (we have experiments for this).
% \item For this to be used during training with little overhead, we also need to set a hyperparameter $E$ to determine when to do this operation. The performance is relatively insensitive to $E$ so long as we are using large learning rates.
% \end{itemize}

% \subsection{Hyperparameters}
% \begin{itemize}
% \item $p$, which is the percentile for the ``noise distribution'', it tries to control the recall for classification.
% \item $E$, which is the epoch at which we perform classification
% \item $p = 10$ is almost always optimal for all cases.
% \item For CIFAR with stepwise, we set $E = $ whenever the lr decays, for cosine we set $E = 50$ if there is noise and $E = 100$ if there is no noise.
% \item For ImageNet, we set $E = 60$.
% \end{itemize}


\begin{table}[htbp]
\small
\begin{center}
\caption{Minimum validation error throughout training (in percentage) on CIFAR10.}
\label{tab:cifar-val}
\begin{tabular}{c|ccc|ccc|c}
\toprule
\multirow{2}{*}{Method} & \multicolumn{3}{|c|}{$\%$ of Mislabeled Examples} & \multicolumn{3}{|c|}{$\%$ of Mislabeled Examples} & \multirow{2}{*}{Network}
\\
                                             & 0                              & 20                              & 40                & 0 & 20 & 40            &   \\\midrule
 \textsc{Oracle}                                      & - & $4.25 \pm 0.05$  & $5.06 \pm 0.05$  & \multirow{4}{*}{WRN-28-10} \\
\textsc{ERM}                                           & $3.73 \pm 0.13$ & $11.53 \pm 0.06$ & $15.57 \pm 0.45$ &  \\
\textsc{NC}                              & $3.80 \pm 0.10$ & $\textbf{5.33} \pm 0.04$  & $\textbf{7.16} \pm 0.20$  &    \\
\textit{mixup}                                                &           $\textbf{3.04} \pm 0.05$     & $6.09 \pm 0.27$ & $9.26 \pm 0.14$  &  \\\midrule
\textsc{GCE}     &            -                    & $10.13 \pm 0.20$                               & $12.87 \pm 0.22$                              & ResNet-34
                                                   \\\midrule
\textsc{MentorNet}             &             -                   & 9                               & 23                              & WRN-101-10
                                                   \\\midrule
\textsc{Ren}$^\star$                   &            -                    &                 -                & $13.08 \pm 0.19$   & WRN-28-10 \\\midrule
\textsc{MentorNet}$^\star$ &       -                         & 8                               & 11   & WRN-101-10 \\\bottomrule                          
\end{tabular}
\end{center}
\end{table}

==> proofs.tex <==
\section{Proof of Theorem \ref{thm:1}}


\begin{customthm}{1}
\label{thm:1}
Suppose we have $N$ training examples $(x_i,y_i)\in\bb R^d\times\{\pm 1\}$  iid from distribution $\mc D$. Suppose the distribution $\mc D$ satisfies that for every $x_i=(x_{i,1},x_{i,2},\cdots,x_{i,d})$ , we have $x_{i,1}=y_i$ and $x_{i,j}$ is independently from $\mc N\left(0,\frac{\lambda^2}{d-1}\right)$ for $2\leq j\leq N$, where $\lambda$ is a positive constant. Suppose we randomly choose $n$ training examples and flip their labels (flip the sign of $y_i$), where $1\leq n< N/2$. Now we have $n$ mislabeled examples and $m=N-n$ correct examples in the training set. Suppose we train a linear classifier $f_w(x)=w^\top x$ using Stochastic Gradient Descent on the objective $\sum_{i=1}^N\ell(y_if_w(x_i))$ using constant learning rate $\eta$, where the loss function $\ell(\cdot)$ is the logistic loss $\ell(z)=\ln(1+\exp(-z))$, and get iterate $w_t$ after iteration $t$. Assume each epoch consists of $K$ iterations each corresponding to a minibatch of size $N/K$, and in each epoch every training example is selected in exactly one minibatch. Then, for $\eta = O\left(\left ((N+\lambda^2)\left(mn/\lambda^2 + N + K\sqrt{mn/\lambda^2 + N}\right)\right)^{-1}\right), d=\Omega\left(\left(\frac{N(m+\lambda^2)}{\min\{2n+\lambda^2,m-n\}}\right)^2\log (N/\delta)\right)$, and any initialization $w_0$, with  probability at least $1-\delta$ over the randomness of the training set,  there exists $T>0$ such that for all $t>T$, it holds that 
\begin{equation*}
    \min_{i:(x_i,y_i)\text{ is mislabeled}}\ell(y_if_{w_t}(x_i))>\max_{j:(x_j,y_j)\text{ is correct}}\ell(y_jf_{w_t}(x_j)).
\end{equation*}
\end{customthm}
Before proving Theorem \ref{thm:1}, we first prove the following three lemmas (Lemma \ref{lm:sgd_max_margin}, \ref{lm:sgdratio} and \ref{lm:lossdual}). Many of the proof techniques for Lemma \ref{lm:sgd_max_margin} are adapted from \citep{soudry2017implicit} and \citep{nacson2018stochastic}.
\begin{lemma}
\label{lm:sgd_max_margin}
Suppose we have $N$ training examples, $(x_1,y_1),(x_2,y_2),\cdots,(x_N,y_N)\in\bb R^d\times\{\pm 1\}$. Assume $x_1,x_2,\cdots,x_N$ are linearly independent. Suppose we train a linear model $f_w(x)=w^\top x$ using Stochastic Gradient Descent on the objective $\sum_{i=1}^N\ell(y_if_w(x_i))$ using constant learning rate $\eta$, where the loss function $\ell(\cdot)$ is the logistic loss $\ell(z)=\ln(1+\exp(-z))$, and get iterate $w_t$ after iteration $t$. Assume each epoch consists of $K$ iterations each corresponding to a minibatch of size $B=N/K$, and in each epoch every training example is selected in exactly one minibatch.  
% We define $\gamma(w)$ to be the margin of $w$ on the training set: $\gamma(w)=\min_{1\leq i\leq N}y_if_w(x_i)$, and $\hat w$ to be the max-margin solution: $\hat w = \argmin\{\|w\|_2:\gamma(w)\geq 1\}$. 
Define $X=[y_1x_1,y_2x_2,\cdots,y_Nx_N]\in\bb R^{d\times N}$. Then, there exists a unique $\bm \alpha = (\alpha_1,\alpha_2,\cdots,\alpha_N)^\top \in\bb R^N$ such that $X^\top X\bm\alpha = (1,1,\cdots,1)^\top$. Moreover, if every $\alpha_i$ is positive and
\begin{equation}
\label{eq:small_rate}
    \eta < \min\left\{\frac 1{2K\beta\sigma_{\max}^2(X)}, \frac {\gamma^*}{2\beta\sigma^3_{\max}(X)(K+\sigma_{\max}(X)/\gamma^*)}\right\},
\end{equation}
where $\gamma^*=\left(\sum_{i=1}^N\alpha_i\right)^{-1/2}$ is the maximum normalized margin and $\beta = \frac 14$ is the smoothness coefficient of $\ell(\cdot)$, then for any initialization $w_0\in\bb R^d$, there exists $\tilde w\in\bb R^d$ satisfying $\forall i,\exp(-y_i\tilde w^\top x_i)=\frac{\alpha_i}\eta$ and 
\begin{equation*}
    \lim\limits_{t\rightarrow +\infty}\left\|w_t-\ln\left(\frac tK\right)\hat w-\tilde w\right\|_2=0,
\end{equation*}
where $\hat w = X\bm\alpha$.

% Assume the examples are linearly separable with max-margin solution $\hat w\neq \mathbf 0$ and corresponding dual solutions $\alpha_1,\alpha_2,\cdots,\alpha_m\in\bb R_{> 0}$ satisfying $\sum_{i=1}^m\alpha_iy_ix_i=\hat w$. Note that here we assume $\alpha_i>0$ for every $i$, which implies every example $(x_i,y_i)$ is a ``support vector'', i.e., $y_i\hat w^\top x_i=1$. Let $\ell(w;x,y)=\ell(yw^\top x)=\ln(1+\exp(-yw^\top x))$ be the Logistic loss. Suppose $w_0\in\bb R^d$ is any initialized weight. For any $t\in\bb N^*$, at time step $t$, we update $w_{t-1}$ to $w_t$ using Stochastic Gradient Descent with batch $B(t)\subseteq \{1,2,\cdots,m\}$:
% \begin{equation}
% \label{eq:sgd_update}
%     w_t=w_{t-1} - \eta\sum\limits_{i\in B(t)}\nabla_w\ell(w_{t-1};x_i,y_i).
% \end{equation}
% Here $\eta\in\bb R_{>0}$ is the learning rate. Suppose each epoch has $K$ iterations, and for every $p\in\bb N^*$, $B(pK-K+1),B(pK-K+2),\cdots,B(pK)$ form a partition of $\{1,2,\cdots,m\}$. Assume the learning rate satisfies
% \begin{equation*}
%     \eta < \min\{\frac 1{2K\beta\sigma_{\max}^2}, \frac r{2\beta\sigma^3_{\max}(K+r ^{-1}\sigma_{\max})}\},
% \end{equation*}
% where $r = \frac 1{\|\hat w\|}$, $\beta$ is the smoothness coefficient of the Logistic loss and $\sigma_{\max}$ is the maximum singular value of the matrix $[x_1,x_2,\cdots,x_m]\in\bb R^{d\times m}$.

% Then, there exist $\tilde w\in\bb R^d$ satisfying $\forall i,\exp(-y_i\tilde w^\top x_i)=\frac{\alpha_i}{\eta}$ and
% \begin{equation*}
%     \lim\limits_{t\rightarrow +\infty}\left\|w_t-\ln\left(\frac tK\right)\hat w-\tilde w\right\|=0
% \end{equation*}
\end{lemma}

\begin{proof}
Since $x_1,x_2,\cdots,x_N$ are linearly independent, $X$ has full column rank and $X^\top X$ is invertible. This proves the existence and uniqueness of $\bm\alpha$. Let's now focus on the case where every $\alpha_i$ is positive and the learning rate satisfies (\ref{eq:small_rate}).

Consider the following hard-margin SVM problem:
\begin{align*}
    \text{Minimize }&\frac 12\|w\|_2^2,\\
    \text{s.t. }&\forall 1\leq i\leq N, y_iw^\top x_i\geq 1.
\end{align*}
By definition, $X^\top \hat w=X^\top X\bm\alpha = (1,1,\cdots,1)^\top$. Therefore, $\hat w$ is a feasible solution to the above optimization problem with objective value $\frac 12\|\hat w\|_2^2=\frac 12\hat w^\top \hat w=\frac 12\bm\alpha^\top X^\top X\bm\alpha=\frac 12\bm\alpha^\top (1,1,\cdots,1)^\top=\frac 12\sum_{i=1}^N\alpha_i$. Moreover, $\bm\alpha$ is a feasible solution to the dual:
\begin{align*}
    \text{Maximize }&\sum_{i=1}^N\alpha_i-\frac 12\sum_{i=1}^N\sum_{j=1}^N\alpha_i\alpha_jy_iy_jx_i^\top x_j,\\
    \text{s.t. }&\forall 1\leq i\leq N,\alpha_i\geq 0,
\end{align*}
with objective value $\sum_{i=1}^N\alpha_i-\frac 12\bm\alpha^\top X^\top X\bm\alpha=\sum_{i=1}^N\alpha_i-\frac 12\bm\alpha^\top (1,1,\cdots,1)^\top=\frac 12\sum_{i=1}^N\alpha_i$. Therefore, $\hat w$ is the global optimum of the primal and $\bm\alpha$ is the global optimum of the dual. By complementary slackness, every $\alpha_i$ being positive means every training example being a support vector. Moreover, $\gamma^* = \left(\sum_{i=1}^N\alpha_i\right)^{-1/2} = \|\hat w\|_2^{-1}$ equals to the maximum normalized margin $\max_{\|w\|_2 = 1}\min_{1\leq i\leq N}y_iw^\top x_i$.

Now let's show that we can assume $w_0\in\Span(x_1,x_2,\cdots,x_N)$ without loss of generality. Otherwise, say $w_0=w^\perp+w_0'$ where $w_0'\in\Span(x_1,x_2,\cdots,x_N)$ and $w^\perp \perp \Span(x_1,x_2,\cdots,x_N)$. Then, the SGD update rule ensures that for every $t$, $w_t=w^\perp + w_t'$ where $w_t'\in\Span(x_1,x_2,\cdots,x_N)$. Moreover, the sequence $w_t'$ also follows the SGD update rule. If we could prove the lemma for $w_0'$, i.e., there exists $\tilde w'\in\bb R^d$ satisfying $\forall i,\exp(-y_i(\tilde w')^\top x_i)=\frac{\alpha_i}{\eta}$ and $\lim\limits_{t\rightarrow +\infty}\|w_t'-\ln(\frac tK)\hat w - \tilde w'\|_2=0$, then taking $\tilde w=\tilde w'+w^\perp$ yields a proof for $w_0$.

Now we assume $w_0\in\Span(x_1,x_2,\cdots,x_N)$ without loss of generality. Note that we have assumed $x_1,x_2,\cdots,x_N$ to be linearly independent, so there exists a unique $\tilde w\in\Span(x_1,x_2,\cdots,x_N)$ satisfying $\forall i,\exp(-y_i\tilde w^\top x_i)=\frac{\alpha_i}{\eta}$. Now we only need to show that $\lim\limits_{t\rightarrow +\infty}\|w_t-\ln(\frac tK)\hat w-\tilde w\|_2=0$.

Note that we can also assume $y_i=1$ for $1\leq i\leq N$ without loss of generality by replacing $y_ix_i$ by a new $x_i$. Define $B(u)$ to be the set of indices of training examples selected in the minibatch corresponding to the $u$th iteration. By Lemma 5 in \cite{nacson2018stochastic}, we know that $\ln(\frac tK)\hat w=K\sum\limits_{u=1}^{t-1}\frac 1u\sum\limits_{n\in B(u)}\alpha_nx_n-\gamma \hat w+o(1)$ as $t\rightarrow +\infty$, where $\gamma$ is the Euler-Mascheroni constant. %where $\|m_4(t)\|=o(t^{-0.5})$. 
Therefore, we only need to show that $\lim\limits_{t\rightarrow +\infty}\|r(t)\|_2=0$, where 
\begin{equation*}
    r(t)=w_t-K\sum\limits_{u=1}^{t-1}\frac 1u\sum\limits_{n\in B(u)}\alpha_nx_n+\gamma\hat w-\tilde w.
\end{equation*}

In Section B.1, \citet{nacson2018stochastic} showed that $\sum_{t=0}^{+\infty}\|r(t+1)-r(t)\|_2^2<\infty$. Lemma 6 in \cite{nacson2018stochastic} showed that there exist $c_1,\delta>0$ such that for all $t\in\bb N^*$, it holds that
\begin{equation*}
    (r(t+1)-r(t))^\top r(t)\leq c_1t^{-1-\delta}.
\end{equation*}
Therefore, $\forall \varepsilon > 0$, we can find $t_1\in\bb N^*$ such that $\forall t',t''\in\bb N^*\text{ with }t''>t'\geq t_1$,
\begin{align}
&\|r(t'')\|_2^2-\|r(t')\|_2^2\nonumber \\
   =&\sum\limits_{t=t'}^{t''-1}(\|r(t+1)\|_2^2-\|r(t)\|_2^2)\nonumber \\
  =&\sum\limits_{t=t'}^{t''-1}(\|r(t+1)-r(t)\|_2^2+2(r(t+1)-r(t))^\top r(t))\nonumber \\
  \leq &\sum\limits_{t=t'}^{t''-1}\|r(t+1)-r(t)\|_2^2+2c_1\sum\limits_{t=t'}^{t''-1}t^{-1-\delta}\nonumber \\
  \leq & \varepsilon.  \label{eq:partialsum}
\end{align}

Now we show that there exist $c_2>0$ and $t_2\in\bb N^*$ such that for all $t\geq t_2$ with $\|r(t)\|_2\geq \varepsilon$, there exists $t'\in\bb N^*$ with $t\leq t'<t+2K$ satisfying $(r(t'+1)-r(t'))^\top r(t')\leq -c_2t^{-1}$. Note that $x_1,\cdots,x_N$ are linearly independent, so $X^\top$ has a minimum positive singular value $\sigma_{\min}:=\min_{r\in\Span\{x_1,\cdots,x_N\}:\|r\|_2=1}\|X^\top r\|_2>0$ and thus
$\|X^\top r(t)\|_2\geq \sigma_{\min}\|r(t)\|_2\geq \sigma_{\min}\varepsilon$.
Therefore, there exists $i_1$ such that 
$|x_{i_1}^\top r(t)|\geq \varepsilon_1:=\frac{\sigma_{\min} \varepsilon}{\sqrt N}$.
By picking $t_2$ sufficiently large, we can ensure that for every $t\geq t_2$, it holds that $\|r(t+1)-r(t)\|_2\leq \frac{\varepsilon_1}{4K(\max_{1\leq i\leq N}\|x_i\|_2)}$. Then, $\forall t'\in\bb N^*$ with $t\leq t'<t+2K$, we have $|x_{i_1}^\top r(t')|\geq |x_{i_1}^\top r(t)|-|x_{i_1}^\top (r(t)-r(t'))|\geq \varepsilon_1-\|x_{i_1}\|_2\|r(t)-r(t')\|_2\geq \frac{\varepsilon_1} 2$. Pick $t'$ so that $i_1\in B(t')$. In Section B.2, \citet{nacson2018stochastic} showed that
\begin{equation}
\label{eq:decomposition}
    (r(t'+1)-r(t'))^\top r(t')\leq \sum\limits_{i\in B(t')}\alpha_i\frac K{t'}(\gamma_i(t')\exp(\tilde m_i(t')-x_i^\top r(t'))-1)x_i^\top r(t')
\end{equation}
as long as we pick $t_2$ sufficiently large, where $\tilde m_i(t)\rightarrow 0$ and $\gamma_i(t)\rightarrow 1$ as $t\rightarrow +\infty$. In Section B.2, \citet{nacson2018stochastic} also showed that there exist $c',\delta'\in\bb R_{>0}$ independent of $t,t'$ such that $\forall 1\leq i\leq N$
\begin{equation}
\label{eq:positive}
    \alpha_i\frac K{t'}(\gamma_i(t')\exp(\tilde m_i(t')-x_i^\top r(t'))-1)x_i^\top r(t')\leq c'(t')^{-1-\delta'}\leq c't^{-1-\delta'}.
\end{equation}
Now we show that there exists $c_2'\in\bb R_{>0}$ independent of $t,t'$ such that 
\begin{equation}
\label{eq:negative}
    \alpha_{i_1}\frac K{t'}(\gamma_{i_1}(t')\exp(\tilde m_{i_1}(t')-x_{i_1}^\top r(t'))-1)x_{i_1}^\top r(t')\leq -c_2'(t')^{-1}\leq -c_2'(t+2K)^{-1}.
\end{equation}
When $x_{i_1}^\top r(t')\geq \frac{\varepsilon_1}{2}$, as long as we pick $t_2$ sufficiently large, we can make sure that $\gamma_{i_1}(t')\exp(\tilde m_{i_1}(t')-x_{i_1}^\top r(t'))-1\leq -\frac{\varepsilon_1}{4}$, so the left hand side of (\ref{eq:negative}) is upper bounded by $-\alpha_{i_1}\frac K{t'}\frac{\varepsilon_1^2}{8}$. Similarly, when $x_{i_1}^\top r(t')\leq -\frac{\varepsilon_1}{2}$, as long as we pick $t_0$ sufficiently large, we can make sure that $\gamma_{i_1}(t')\exp(\tilde m_{i_1}(t')-x_{i_1}^\top r(t'))-1\geq \frac{\varepsilon_1}{4}$, so the left hand side of (\ref{eq:negative}) is again upper bounded by $-\alpha_{i_1}\frac K{t'}\frac{\varepsilon_1^2}{8}$. Therefore, we can choose $c_2'=(\min_{1\leq i\leq N}\alpha_{i})K\varepsilon_1^2/8$.

Combining (\ref{eq:positive}) and (\ref{eq:negative}) with (\ref{eq:decomposition}), we know
\begin{equation*}
    (r(t'+1)-r(t'))^\top r(t')\leq |B(t')|c't^{-1-\delta'}-c_2'(t+2K)^{-1}\leq c'Nt^{-1-\delta'}-c_2'(t+2K)^{-1}.
\end{equation*}
Now as long as we pick $t_2$ sufficiently large, we know there exists $c_2>0$ independent of $t,t'$ such that $(r(t'+1)-r(t'))^\top r(t')\leq -c_2t^{-1}$.

Suppose $\|r(t)\|_2\geq\varepsilon$ for all $t\geq \max\{t_1,t_2\}$. Then 
\begin{align*}
&\sum\limits_{t\geq \max\{t_1,t_2\}}(\|r(t+1)\|_2^2-\|r(t)\|_2^2)\\
=&\sum\limits_{t\geq \max\{t_1,t_2\}}\|r(t+1)-r(t)\|_2^2+2\sum\limits_{t\geq \max\{t_1,t_2\}}(r(t+1)-r(t))^\top r(t)\\
\leq &\varepsilon+2c_1\sum\limits_{t\geq \max\{t_1,t_2\}}t^{-1-\delta}-2c_2\sum\limits_{t\geq \max\{t_1,t_2\}\atop t\text{ is a multiple of }2K}t^{-1}\\
=&-\infty,
\end{align*}
a contradiction. Therefore, there exists $t_3\geq \max\{t_1,t_2\}$ with $\|r(t_3)\|_2\leq \varepsilon$. Now for any $t\geq t_3$, we have $\|r(t)\|_2^2\leq \varepsilon^2+\varepsilon$ according to (\ref{eq:partialsum}). By the arbitrariness of $\varepsilon>0$, we have proved $\lim\limits_{t\rightarrow +\infty}\|r(t)\|_2=0$.
\end{proof}
\begin{lemma}
\label{lm:sgdratio}
% Suppose we have $N$ training examples $(x_1,y_1),(x_2,y_2),\cdots,(x_N,y_N)\in\bb R^d\times\{\pm 1\}$ and assume $(x_i)_{1\leq i\leq N}$ are linearly independent. Suppose we train a linear model $f_w(x)=w^\top x$ using Stochastic Gradient Descent on the objective $\sum_{i=1}^N\ell(y_if_w(x_i))$ using constant learning rate $\eta$, where the loss function $\ell(\cdot)$ is the logistic loss $\ell(z)=\ln(1+\exp(-z))$, and get iterate $w_t$ after iteration $t$. Assume each epoch consists of $K$ iterations, and in each epoch every training example is selected exactly once. We define $\gamma(w)$ to be the margin of $w$ on the training set: $\gamma(w)=\min_{1\leq i\leq N}y_if_w(x_i)$, and the max-margin solution $\hat w$ be $\argmin\{\|w\|_2:\gamma(w)\geq 1\}$. Let $\alpha_1,\alpha_2,\cdots,\alpha_N\in\bb R_{\geq 0}$ be the coefficient of the linear expression of $\hat w$ by $y_1x_1,y_2x_2,\cdots,y_Nx_N$, i.e., $\hat w = \sum_{i=1}^N\alpha_iy_ix_i$. Then,
In the setting of Lemma \ref{lm:sgd_max_margin}, we have
$\forall 1\leq i\leq N$,
\begin{equation*}
    \lim\limits_{t\rightarrow +\infty}\frac{\ell(y_if_{w_t}(x_i))}{\sum_{j=1}^N\ell(y_jf_{w_t}(x_j))}=\frac{\alpha_i}{\sum_{j=1}^N\alpha_j}.
\end{equation*}


\end{lemma}
\begin{proof}
Theorem 1 in \citep{nacson2018stochastic} showed that $\forall 1\leq i\leq N, f_{w_t}(x_i)\rightarrow +\infty$ as $t\rightarrow +\infty$, so $\lim\limits_{t\rightarrow +\infty}\frac{\ell(y_if_{w_t}(x_i))}{\exp(-y_iw_t^\top x_i)}=1$, which implies $\lim\limits_{t\rightarrow +\infty}\frac{\sum_{j=1}^N\ell(y_jf_{w_t}(x_j))}{\sum_{j=1}^N\exp(-y_jw_t^\top x_j)}=1$. Therefore, we only need to show that $\lim\limits_{t\rightarrow +\infty}\frac{\exp(-y_iw_t^\top x_i)}{\sum_{j=1}^N\exp(-y_jw_t^\top x_j)}=\frac{\alpha_i}{\sum_{j=1}^N\alpha_j}$. According to Lemma \ref{lm:sgd_max_margin}, we have $w_t=\ln\left(\frac tK\right)\hat w+\tilde w + o(1)$. Note that $y_i\hat w^\top x_i=1,\exp(-y_i\tilde w^\top x_i)=\frac{\alpha_i}{\eta}$, we have
\begin{align*}
    &\lim\limits_{t\rightarrow +\infty}\frac{\exp(-y_iw_t^\top x_i)}{\sum_{j=1}^N\exp(-y_jw_t^\top x_j)}\\
    =&\lim\limits_{t\rightarrow +\infty}\frac{\exp(-y_i\ln(\frac tK)\hat w^\top x_i)\exp(-y_i\tilde w^\top x_i)\exp(o(1))}{\sum_{j=1}^N\exp(-y_j\ln(\frac tK)\hat w^\top x_j)\exp(-y_j\tilde w^\top x_j)\exp(o(1))}\\
    =&\lim\limits_{t\rightarrow +\infty}\frac{(\frac tK)^{-1}\cdot \frac{\alpha_i}{\eta}\exp(o(1))}{\sum_{j=1}^N(\frac tK)^{-1}\cdot \frac{\alpha_j}{\eta}\exp(o(1))}\\
    =&\lim\limits_{t\rightarrow +\infty}\frac{\alpha_i\exp(o(1))}{\sum_{j=1}^N\alpha_j\exp(o(1))}\\
    =&\frac {\alpha_i}{\sum_{j=1}^N\alpha_j}.
\end{align*}
\end{proof}
\begin{lemma}
\label{lm:lossdual}
In the setting of Theorem \ref{thm:1}, with probability at least $1-\delta$, the following are true:
\begin{enumerate}
	\item Define $X = [y_1x_1,y_2x_2,\cdots,y_Nx_N]\in\bb R^{d\times N}$. Then, $\sigma_{\max}(X)\leq \sqrt{N+2\lambda ^2}$;
	\item There exists $\bm\alpha = (\alpha_1,\alpha_2,
	\cdots,\alpha_N)^\top \in\bb R_{>0}^N$ such that $X^\top X\bm\alpha=(1,1,\cdots,1)^\top$;
	\item $\max_{1\leq i \leq N, (x_i,y_i)\text{ is correct}}\alpha_i<\min_{1\leq i\leq N, (x_i,y_i)\text{ is mislabeled}}\alpha_i$;
	\item $\frac 12\sqrt{\frac{4mn + \lambda^2N}{\lambda^2(N+\lambda^2)}}\leq \sqrt{\sum_{i=1}^N\alpha_i}\leq 2\sqrt{\frac{4mn + \lambda^2N}{\lambda^2(N+\lambda^2)}}$.
\end{enumerate}
\end{lemma}





\begin{proof}[Proof of Lemma \ref{lm:lossdual}]
We can rearrange the indices so that $(x_i,y_i)$ are correct for $1\leq i\leq m$ and mislabeled for $m < i\leq N$. Without loss of generality, we can assume $y_i = 1$ for all $1\leq i\leq N$ by always replacing $y_ix_i$ by a new $x_i$. Now we have $x_{i,1}=1$ for $1\leq i\leq m$ and $x_{i,1}=-1$ for $m < i\leq N$. Note that $\frac {d-1}{\lambda^2}(x_i^\top x_i-1)$ is of distribution $\chi^2(d-1)$, a sum of $d-1$ iid sub-exponential $(4,4)$ random variables each with mean $1$. By the concentration results for sub-exponential random variables, we have
\begin{equation*}
    \Pr\left[\left|\frac{d-1}{\lambda^2}(x_i^\top x_i-1)-(d-1)\right|\geq\varepsilon(d-1)\right]\leq 2\exp\left(-\frac{\varepsilon^2(d-1)}{8}\right), \forall 0\leq \varepsilon \leq 1.
\end{equation*}
Similarly, when $1\leq i<j\leq N$, $\frac{d-1}{\lambda^2}(x_i^\top x_j-x_{i,1}x_{j,1})$ is a sum of $(d-1)$ iid sub-exponential $(2,2)$ random variables each with mean zero, so we have
\begin{equation*}
    \Pr\left[\left|\frac{d-1}{\lambda^2}(x_i^\top x_j-x_{i,1}x_{j,1})\right|\geq \varepsilon(d-1)\right]\leq 2\exp\left(-\frac{\varepsilon^2(d-1)}{4}\right),\forall 0\leq \varepsilon \leq 1.
\end{equation*}
%Define $\bm\alpha=(\alpha_1,\alpha_2,\cdots,\alpha_m,\beta_1,\beta_2,\cdots,\beta_n)^\top\in\bb R^{m+n}$. 
Define $A=(A_{ij})\in\bb R^{N\times N}$ such that $\forall 1\leq i\leq N,A_{ii}=1+\lambda^2,\forall 1\leq i<j\leq m,A_{ij}=A_{ji}=1,\forall m<i<j\leq N,
A_{ij}=A_{ji}=1,\forall 1\leq i\leq m<j\leq N,A_{ij}=A_{ji}=-1$. By the Union Bound, the above concentration results imply that $\forall 0\leq \varepsilon \leq 1$, with probability at least $1-2N^2\exp(-\frac{\varepsilon^2(d-1)}{8})$, every entry in $X^\top X$ differs from its corresponding entry in $A$ by at most $\varepsilon \lambda^2$.  As a consequence, with at least the probability, $\|X^\top X-A\|_\infty < \varepsilon\lambda^2N$, $\|X^\top X-A\|_1<\varepsilon \lambda^2N$ and $\|X^\top X-A\|_2\leq \|X^\top X-A\|_F<\varepsilon \lambda^2N$,  
where $\|\cdot\|_\infty,\|\cdot\|_1$ and $\|\cdot\|_2$ are the operator norm induced by $L_\infty$, the operator norm induced by $L_1$ and the spectral norm, respectively.
Let's choose \begin{equation*}\varepsilon=\frac{(N+\lambda^2)}{2(2N-2+\lambda^2)N}\cdot\frac{\min\{2n + \lambda^2,m-n\}}{2m + \lambda^2}\in (0,1/N]\subseteq (0,1).
\end{equation*}

Now, combining $\|X^\top X-A\|_2 < \varepsilon \lambda^2N\leq \lambda^2$ and $\|A\|_2=N+\lambda^2$ gives $\|X^\top X\|_2\leq N + 2\lambda^2$. Therefore, $\sigma_{\max}(X)\leq \sqrt{N + 2\lambda^2}$. Note that the success probability $1-2N^2\exp(-\frac{\varepsilon^2(d-1)}{8})$ is at least $1-\delta$ by restraining $d\geq 2000\left(\frac{N(m+\lambda^2)}{\min\{2n+\lambda^2,m-n\}}\right)^2\log\frac N\delta$. 


Note that the inverse of $A$ is $A^{-1}=(A^{-1}_{ij})\in\bb R^{N\times N}$ with $\forall 1\leq i\leq N,A^{-1}_{ii}=\frac{1}{\lambda^2}-\frac{1}{\lambda^2(N+\lambda^2)},\forall 1\leq i<j\leq m,A^{-1}_{ij}=A^{-1}_{ji}=-\frac{1}{\lambda^2(N+\lambda^2)},\forall m<i<j\leq N,A^{-1}_{ij}=A^{-1}_{ji}=-\frac{1}{\lambda^2(N+\lambda^2)},\forall 1\leq i\leq m<j\leq N,A^{-1}_{ij}=A^{-1}_{ji}=\frac{1}{\lambda^2(N+\lambda^2)}$. Therefore, $\|A^{-1}\|_\infty=\frac{2N-2+\lambda^2}{\lambda^2(N+\lambda^2)}$, which implies that $\min_{z\in\bb R^{N}:\|z\|_\infty=1}\|Az\|_\infty=\frac{\lambda^2(N+\lambda^2)}{2N-2+\lambda^2}$. Therefore, $\min_{z\in\bb R^{N}:\|z\|_\infty=1}\|X^\top Xz\|_\infty\geq  \frac{\lambda^2(N+\lambda^2)}{2N-2+\lambda^2} - \|X^\top X-A\|_\infty > \frac{\lambda^2(N+\lambda^2)}{2N-2+\lambda^2}-\varepsilon\lambda^2N>0$ and thus $X^\top X$ is invertible and 
\begin{equation*}\|(X^\top X)^{-1}\|_\infty< \left(\frac{\lambda^2(N+\lambda^2)}{2N-2+\lambda^2}-\varepsilon\lambda^2N\right)^{-1}.
\end{equation*}
Define 
\begin{equation*}
\rvc=\left(\underbrace{\frac{2n+\lambda^2}{\lambda^2(N+\lambda^2)},\cdots, \frac{2n+\lambda^2}{\lambda^2(N+\lambda^2)}}_{m},\underbrace{\frac{2m+\lambda^2}{\lambda^2(N+\lambda^2)},\cdots, \frac{2m+\lambda^2}{\lambda^2(N+\lambda^2)}}_{n}\right)^\top\in\bb R^{N}.
\end{equation*}

% By standard concentration results, $\forall \varepsilon\in(0,1/2)$, with probability at least $1-C_1(m+n)^2\exp(-C_2\varepsilon^2d)$ for universal constants $C_1,C_2$, all of the following are true:
% \begin{enumerate}
% 	\item $\forall 1\leq i\leq N, |x_i^\top x_i-(1+\lambda^2)|< \varepsilon (1+\lambda^2)$;
% 	\item $\forall 1\leq i<j\leq m,|x_i^\top x_j-1|< \varepsilon (1+\lambda^2)$;
% 	\item $\forall m< i<j\leq N,|x_i^\top x_j-1|< \varepsilon (1+\lambda^2)$;
% 	\item $\forall 1\leq i\leq m < j\leq N,|x_i^\top x_j+1|<\varepsilon(1+\lambda^2)$.
% \end{enumerate} 
 


Suppose $\bm\alpha$ is the unique solution to the equation $X^\top X\bm\alpha=(\underbrace{1,\cdots,1}_{N})^\top$. We will prove that $\bm\alpha=(\alpha_1,\alpha_2,\cdots,\alpha_N)^\top$ satisfies statements 2, 3 and 4,
%Define $\hat w=X\bm\alpha$. We have $X^\top\hat w=(\underbrace{1,\cdots,1}_{N})^\top$. Therefore, $\forall i,\hat w^\top x_i=1,\hat w^\top y_i=1$. 
%Moreover, $\|\hat w\|_2^2=\hat w^\top \hat w=\bm\alpha^\top X^\top X\bm\alpha=\bm\alpha^\top (1,\cdots,1)^\top$. 
i.e., $\forall i,\alpha_i>0$ , $\max_{1\leq i\leq m}\alpha_i<\min_{m< i\leq N}\alpha_i$ and $\frac 12\sqrt{\frac{4mn + \lambda^2N}{\lambda^2(N+\lambda^2)}}\leq \sqrt{\sum_{i=1}^N\alpha_i}\leq 2\sqrt{\frac{4mn + \lambda^2N}{\lambda^2(N+\lambda^2)}}$. To show statements 2 and 3, we only need $\|\bm\alpha-\rvc\|_\infty< \min\left\{\frac{2n+\lambda^2}{\lambda^2(N+\lambda^2)},\frac{m-n}{\lambda^2(N+\lambda^2)}\right\}$. Note that $X^\top X\bm\alpha=(\underbrace{1,\cdots,1}_{N})^\top=A\rvc$, and thus $X^\top X(\rvc-\bm\alpha)=(X^\top X-A)\rvc$. Therefore, 
\begin{align}
\|\rvc-\bm\alpha\|_\infty\leq &\|(X^\top X)^{-1}\|_\infty\|(X^\top X-A)\|_\infty \|\rvc\|_\infty\nonumber \\
< &\left(\frac{\lambda^2(N+\lambda^2)}{2N-2+\lambda^2}-\varepsilon\lambda^2 N\right)^{-1}\varepsilon\lambda^2 N\cdot\frac{2m+\lambda^2}{\lambda^2(N+\lambda^2)}.\label{eq:1}
\end{align}
Recall that we chose  $\varepsilon=\frac{(N+\lambda^2)}{2(2N-2+\lambda^2)N}\cdot \frac{\min\{2n+\lambda^2,m-n\}}{2m+\lambda^2}$ which gives the desired $\|\bm\alpha-\rvc\|_\infty<\min\{\frac{2n+\lambda^2}{\lambda^2(N+\lambda^2)},\frac{m-n}{\lambda^2(N+\lambda^2)}\}$. 

Similarly, 
\begin{align*}
\|\rvc-\bm\alpha\|_1\leq & \|(X^\top X)^{-1}\|_1\|(X^\top X-A)\|_1\|\rvc\|_1\\
= &\|(X^\top X)^{-1}\|_\infty\|(X^\top X-A)\|_\infty\|\rvc\|_1\\
< &\left(\frac{\lambda^2(m+n+\lambda^2)}{2m+2n-2+\lambda^2}-\varepsilon\lambda^2 N\right)^{-1}\varepsilon\lambda^2 N\cdot \|\rvc\|_1\\
\leq & \frac 12\|\rvc\|_1.
\end{align*}
Therefore, $\frac 14\cdot \frac{4mn+\lambda^2N}{\lambda^2(N+\lambda^2)}=\frac 14\|\rvc\|_1\leq \|\bm\alpha\|_1\leq 4\|\rvc\|_1=4\cdot \frac{4mn+\lambda^2N}{\lambda^2(N+\lambda^2)}$. Taking the squared root gives $\frac 12\sqrt{\frac{4mn+\lambda^2N}{\lambda^2(N+\lambda^2)}}\leq \sqrt{\sum_{i=1}^N\alpha_i}\leq 2\sqrt{\frac{4mn+\lambda^2N}{\lambda^2(N+\lambda^2)}}$.
\end{proof}
\begin{remark}
Lemma \ref{lm:lossdual} implies that (under the same assumptions) with probability at least $1-\delta$ the optimal normalized margin for the training set is $\max_{\|w\|_2=1}\min_{1\leq i\leq N}y_iw^\top x_i=\frac 1{\|\hat w\|_2}=\frac{1}{\sqrt{\sum_{i=1}^N\alpha_i}}\leq 2\sqrt{\frac{\lambda^2(N+\lambda^2)}{4mn+\lambda^2N}}$, which can be arbitrarily close to zero as the size of the training set grows.
\end{remark}
\begin{proof}[Proof of Theorem \ref{thm:1}]
To combine Lemma \ref{lm:sgdratio} and Lemma \ref{lm:lossdual} to get Theorem \ref{thm:1}, we only need to show that (\ref{eq:small_rate}) holds given the four properties claimed in Lemma \ref{lm:lossdual}. The first and the fourth property imply $\sigma_{\max}(X)\leq \sqrt{N+2\lambda^2}$ and $\gamma^*\geq \frac 12\sqrt{\frac{\lambda^2(N+\lambda^2)}{4mn+\lambda^2N}}$. Therefore, 
\begin{align*}
&\frac {\gamma^*}{2\beta\sigma^3_{\max}(X)(K+\sigma_{\max}(X)/\gamma^*)}\\
\geq &\frac{\frac 12\sqrt{\frac{\lambda^2(N+\lambda^2)}{4mn + \lambda^2N}}}{2\beta(N+2\lambda^2)^{3/2}\left(K+2\sqrt{\frac{4mn+\lambda^2 N}{\lambda^2(N+\lambda^2)}}\cdot\sqrt{N+2\lambda^2}\right)}\\
\geq & \frac 1{16\beta}\cdot\frac{\sqrt{\frac{\lambda^2}{4mn + \lambda^2N}}}{(N+\lambda^2)(K+4\sqrt{\frac{4mn+\lambda^2N}{\lambda^2}})}\\
=&\frac 1{16\beta}\cdot \frac 1{(N+\lambda^2)(K\sqrt{4mn/\lambda^2 + N}+4(4mn/\lambda^2 + N))}\\
\geq &\frac 1{256\beta}\cdot ((N+\lambda^2)(K\sqrt{mn/\lambda^2+N}+mn/\lambda^2+N))^{-1},
\end{align*}
and
\begin{align*}
&\frac 1{2K\beta\sigma_{\max}^2(X)}\\
\geq &\frac 1{2\beta}\cdot \frac {1}{K(N+\lambda^2)}.
\end{align*}
Therefore, the right-hand-side of (\ref{eq:small_rate}) is at least $\frac 1{256\beta}\cdot ((N+\lambda^2)(K\sqrt{mn/\lambda^2+N}+mn/\lambda^2+N))^{-1}$, so restraining $\eta$ from exceeding this quantity satisfies (\ref{eq:small_rate}).
\end{proof}
% \begin{remark}
% If we just need every point being a support vector with probability at least $2/3$, then we only need $d=\Omega\left(\frac{(1+\lambda^2)^2(m+n)^2(2m+\lambda^2)^2\log(m+n)}{(2n+\lambda^2)^2\lambda^4}\right)$, which can be ensured by $d=\Omega\left(\frac{(m+n)^2m^2\log(m+n)}{n^2}\right)$ as long as $\lambda = \Omega(1)$. This means that we are allowed to have arbitrarily large $\lambda$ when $d$ is fixed.
% \end{remark}
% Let's try to do a similar analysis using the $L_2$ norm. Similarly to (\ref{eq:1}), we have
% \begin{align*}
% \|\rvc-\bm\alpha\|_2\leq & \|(X^\top X)^{-1}\|_2\|(X^\top X)-A\|_2\|\rvc\|_2\\
% \leq &(\|A^{-1}\|_2^{-1}-\|(X^\top X)-A\|_2)^{-1}\|(X^\top X)-A\|_2\|\rvc\|_2.
% \end{align*}
% Therefore, we can give upper bounds for $\|\rvc-\bm\alpha\|_2$ by showing upper bounds for $\|A^{-1}\|_2,\|(X^\top X)-A\|_2$ and $\|\rvc\|_2$. Here, we use $\|\cdot\|_2$ for matrices to denote the operator norm induced by the $L_2$ norm for vectors, which is the same as the spectral norm. Note that we have $\|\rvc\|_2=\frac{\sqrt{m(2n+\lambda^2)^2+n(2m+\lambda^2)^2}}{\lambda^2(m+n+\lambda^2)}$ and $\|A^{-1}\|_2=\frac 1{\lambda^2}$. Again, with probability at least $1-C_1(m+n)^2\exp(-C_2\varepsilon^2d)$, each entry in $(X^\top X-A)$ has absolute value at most $\varepsilon(1+\lambda^2)$ and thus $\|X^\top X-A\|_2\leq \varepsilon(1+\lambda^2)(m+n)$.\footnote{The bound for $\|X^\top X-A\|_2$ can be improved via random matrix theory. TO DO.} Therefore, we have
% \begin{equation}
% \label{eq:2}
% \|\rvc-\bm\alpha\|_2\leq (\lambda^2-\varepsilon(1+\lambda^2)(m+n))^{-1}\varepsilon(1+\lambda^2)(m+n)\cdot \frac{\sqrt{m(2n+\lambda^2)^2+n(2m+\lambda^2)^2}}{\lambda^2(m+n+\lambda^2)}.
% \end{equation}
% If we want to make sure that at most $s$ fraction of the $n$ mislabeled examples have relatively low dual, we need $\|\rvc-\bm\alpha\|_2\leq \sqrt{sn}\cdot \frac{m-n}{\lambda^2(m+n+\lambda^2)}$. To ensure this from (\ref{eq:2}), we need 
% \begin{equation*}
% \varepsilon\leq \frac{\sqrt{sn}(m-n)\lambda^2}{2(1+\lambda^2)(m+n)\sqrt{m(2n+\lambda^2)^2+n(2m+\lambda^2)^2}}.
% \end{equation*}
% To make the failure probability upper bounded by $1/3$, we set $d=\Omega(\frac{\log(m+n)}{\varepsilon^2})$, i.e.,
% \begin{equation*}
% d=\Omega\left(\frac{(1+\lambda^2)^2(m+n)^2(m(2n+\lambda^2)^2+n(2m+\lambda^2)^2)\log(m+n)}{sn(m-n)^2\lambda^4}\right).
% \end{equation*}
% Unfortunately, this bound is no better than the bound we obtained using the infinity norm, even when $s$ is large (say $s=\Theta(1)$).
\section{Theorem for Section 3.2}
The following definition follows that given in \citep{wei2018margin}.
\begin{definition}[$a$-positive-homogeneous functions] We say $g:\bb R^{d_1}\rightarrow \bb R^{d_2}$ is $a$-positive-homogeneous for $a\in\bb R$ if $\forall c> 0,\forall w\in\bb R^{d_1}, g(cw)=c^ag(w)$.

\end{definition}
\begin{theorem}
\label{thm:loss_separation_deep}
Suppose we have $N$ training examples $(x_i,y_i)\in\bb R^{d_0}\times\{1,2,\cdots, K\}$ for $1\leq i\leq N$.  Suppose we train a classifier $f_w(x)\in\bb R^K$ with weights $w\in\bb R^d$.
% that takes $x\in\bb R^{d_0}$ and predicts its label $\hat y = \argmax_{1\leq i\leq K}f_w(x)[i]$. 
Suppose $f_w(x)$ is a continuously differentiable and $a$-positive-homogeneous function of $w$ for $a>0$, for example a deep network activated by $(\mathrm{ReLU}(\cdot))^{1.01}$. Let $w_\lambda\in\argmin\sum_{i=1}^N\ell(f_w(x_i),y_i)+\lambda\|w\|_2^2$, where the loss function $\ell(\cdot,\cdot)$ is the cross-entropy loss: $\ell(z,y)=-\ln(\frac{\exp(z[y])}{\sum_{1\leq j\leq K}\exp(z[j])})$. We define $\gamma(w)$ to be the margin of $w$ on the training set: $\gamma(w)=\min_{1\leq i\leq N, 1\leq j\leq K, j\neq y_i}(f_w(x_i)[y_i]-f_w(x_i)[j])$. Assume the training set is separable, i.e., there exists $w\in\bb R^d$ such that $\gamma(w)>0$. Suppose as $\lambda$ approaches $0^+$, $w_\lambda$ converges in direction to a max-margin solution $\hat w\in \argmin\{\|w\|_2:\gamma(w)\geq 1\}$. Assume $(\nabla_wf_w(x_i)[j]|_{w=\hat w})_{1\leq i\leq N,1\leq j\leq K}$ are linearly independent. Then $\hat w$ can be expressed as a linear combination of $(\nabla_wf_w(x_i)[j]|_{w=\hat w})_{1\leq i\leq N,1\leq j\leq K}$. Moreover, suppose $(\alpha_{i,j})_{1\leq i\leq N,1\leq j\leq K}\in\bb R^{N\times K}$ are the coefficients, i.e., $\hat w =\sum_{i=1}^N\sum_{j=1}^L\alpha_{i,j}\nabla_wf_w(x_i)[j]|_{w=\hat w}$, then
\begin{equation*}
    \lim\limits_{t\rightarrow +\infty}\frac{\ell(f_{w_t}(x_i),y_i)}{\sum_{j=1}^N\ell(f_{w_t}(x_j),y_j)}=\frac{\alpha_{i,y_i}}{\sum_{j=1}^N\alpha_{j,y_j}}.
\end{equation*}
\end{theorem}
% Suppose we have a sample of $m$ examples, $(x_1,y_1),(x_2,y_2),\cdots,(x_m,y_m)\in\bb R^d\times\{-1,1\}$ where $0<m<d$ (over-parameterized). Assume $x_1,x_2,\cdots,x_m$ are linearly independent. Assume the examples are linearly separable with max-margin solution $\hat w\neq \mathbf 0$ and corresponding dual solutions $\alpha_1,\alpha_2,\cdots,\alpha_m\in\bb R_{\geq 0}$ satisfying $\sum_{i=1}^m\alpha_iy_ix_i=\hat w$. Let $\ell(w;x,y)=\ell(yw^\top x)=\ln(1+\exp(-yw^\top x))$ be the Logistic loss. Suppose $w_\lambda$ is the global optimum of the following optimization problem:
% \begin{equation}
% \label{eq:opt1}
%     \text{Minimize }\sum\limits_{i=1}^m\ell(w;x_i,y_i)+\lambda\|w\|_2 \text{ over }w\in\bb R^d.
% \end{equation}
% Then, for any $1\leq j,k\leq m$ with $\alpha_k>0$, we have
% \begin{equation*}
%     \lim\limits_{\lambda\rightarrow 0^+}\frac{\ell(w_\lambda;x_j,y_j)}{\ell(w_\lambda;x_k,y_k)}=\frac{\alpha_j}{\alpha_k}.
% \end{equation*}

% \begin{proof}
% Since $w_\lambda$ is the global minimum of optimization problem (\ref{eq:opt1}), the gradient of the objective at $w_\lambda$ is zero:
% \begin{equation*}
%     \sum\limits_{i=1}^m\nabla_w\ell(w_\lambda;x_i,y_i)+2\lambda w_\lambda =0.
% \end{equation*}
% According to \cite{rosset2004margin} (Theorem 2.1), $w_\lambda$ direction converges to $\hat w$ as $\lambda$ approaches $0^+$, i.e., there exists $r_\lambda>0$ such that $w_\lambda=r_\lambda\hat w +o(r_\lambda)$ and $r_\lambda\rightarrow +\infty$ as $\lambda\rightarrow 0^+$. Therefore,
% \begin{equation*}
%     \sum\limits_{i=1}^m\nabla_w\ell(w_\lambda;x_i,y_i)+2\lambda r_\lambda \hat w + 2\lambda o(r_\lambda)=0
% \end{equation*}
% Substituting $\hat w = \sum_{i=1}^m\alpha_iy_ix_i$, $\nabla_w\ell(w_\lambda;x_i,y_i)=-(1+\exp(y_iw_\lambda ^\top x_i)^{-1}y_ix_i$ and dividing the equality by $2\lambda r_\lambda$, we get
% \begin{equation*}
%     \sum\limits_{i=1}^m(\alpha_i-\frac{1}{2\lambda r_\lambda}\cdot(1+\exp(y_iw_\lambda^\top x_i)^{-1})y_ix_i=o(1)
% \end{equation*}
% Therefore, noting that $x_i$ are linearly independent, we have $\forall 1\leq i\leq m,\lim\limits_{\lambda\rightarrow 0^+}\frac{1}{2\lambda r_\lambda}(1+\exp(y_iw_\lambda x_i)^{-1})=\alpha_i$, so
% \begin{equation*}
%     \lim\limits_{\lambda\rightarrow 0^+}\frac{(1+\exp(y_jw_\lambda^\top x_j))^{-1}}{(1+\exp(y_kw_\lambda^\top x_k))^{-1}}=\frac{\alpha_j}{\alpha_k}.
% \end{equation*}
% Finally, we complete the proof by noting that $y_jw_\lambda^\top x_j,y_kw_\lambda^\top x_k\rightarrow +\infty$ as $\lambda \rightarrow 0^+$ (see \cite{rosset2004margin}, Lemma 2.2), which implies $\lim_{\lambda\rightarrow 0^+}\frac{(1+\exp(y_jw_\lambda^\top x_j)^{-1}}{\ell(w_\lambda;x_j,y_j)}=1$ and $\lim_{\lambda\rightarrow 0^+}\frac{(1+\exp(y_kw_\lambda^\top x_k)^{-1}}{\ell(w_\lambda;x_k,y_k)}=1$.
% \end{proof}

% The following lemma can be proved by following the analysis of \cite{soudry2017implicit, nacson2018stochastic}.


% \begin{lemma}
% \label{lm:weakregdeep}
% Suppose we have a sample of $m$ examples, $(x_1,y_1),(x_2,y_2),\cdots,(x_m,y_m)\in\bb R^{d_1}\times\{-1,1\}$. Let $\ell(w;x,y)=\ell(yf_w(x))=\ln(1+\exp(-yf_w(x)))$ be the Logistic loss associated with neural network $f_w(x)\in\bb R$ parameterized by $w\in\bb R^d$. Suppose $d>m$ (over-parameterized). Suppose the neural network is continuously differentiable and positive-homogeneous of order $\sigma>0$ (for example, a neural network with activation function $\mathrm{activation}(z)=(ReLU(z))^{1.01}$). Suppose $w_\lambda$ is one of the global optimizers of the following optimization problem:
% \begin{equation}
% \label{eq:opt2}
%     \text{Minimize }\sum\limits_{i=1}^m\ell(w;x_i,y_i)+\lambda\|w\|_2\text{ over }w\in\bb R^d,
% \end{equation}
% and suppose $w_\lambda$ direction converges to $\hat w$, i.e., there exists $r_\lambda >0$ such that $w_\lambda = r_\lambda\hat w+o(r_\lambda)$ with $r_\lambda\rightarrow +\infty$ as $\lambda \rightarrow 0^+$. Suppose $\hat w$ fits the data perfectly: $\forall 1\leq i\leq m,y_if_{\hat w}(x_i)>0$. Assume $(\nabla_w\ell(\hat w;x_i,y_i))_{1\leq i\leq m}$ are linearly independent. Then there exist $\alpha_1,\alpha_2,\cdots,\alpha_m\in\bb R_{\geq 0}$ satisfying $\sum_{i=1}^m\alpha_iy_i\nabla_wf_{\hat w}(x_i)=\hat w$ and for all $1\leq j,k\leq m$ with $\alpha_k>0$, we have
% \begin{equation*}
%     \lim\limits_{\lambda\rightarrow 0^+}\frac{\ell(w_\lambda;x_j,y_j)}{\ell(w_\lambda;x_k,y_k)}=\frac{\alpha_j}{\alpha_k}.
% \end{equation*}
% \end{lemma}
\begin{proof}
Since $w_\lambda$ optimizes $\sum_{i=1}^N\ell(f_w(x_i),y_i)+\lambda\|w\|_2^2$, the gradient at $w_\lambda$ is zero:
\begin{equation*}
    \sum\limits_{i=1}^N\nabla_w\ell(f_w(x_i),y_i)|_{w=w_\lambda}+2\lambda w_\lambda = 0.
\end{equation*}
Define $\beta_{i,y_i}(w)=\frac{\sum_{1\leq k\leq K,k\neq y_i}\exp(f_{w}(x_i)[k])}{\sum_{1\leq k\leq K}\exp(f_{w}(x_i)[k])}$ and $\beta_{i,j}(w)=-\frac{\exp(f_{w}(x_i)[j])}{\sum_{1\leq k\leq K}\exp(f_{w}(x_i)[k])}$ for $1\leq i\leq N,1\leq j\leq K,j\neq y_i$.
Note that $\nabla_w\ell(f_w(x_i),y_i)=-\sum_{j=1}^K\beta_{i,j}(w)\nabla_wf_w(x_i)[j]$, we have
\begin{equation*}
    -\sum\limits_{i=1}^N\sum\limits_{j=1}^K \beta_{i,j}(w_\lambda)\nabla_wf_{w}(x_i)[j]|_{w=w_\lambda}+2\lambda w_\lambda = 0.
\end{equation*}
Note that $\min_{\|w\|_2=R}\sum_{i=1}^N\ell(f_w(x_i),y_i)\rightarrow 0$ as $R\rightarrow +\infty$, so $\|w_\lambda\|_2\rightarrow +\infty$ as $\lambda\rightarrow 0^+$. Therefore, we can assume $w_\lambda = r_\lambda \hat w + o(r_\lambda)$ for $r_\lambda\rightarrow +\infty$ as $\lambda\rightarrow 0^+$. Note that $\nabla_wf_w(x)$ is $(a-1)$-positive-homogeneous, we know
\begin{equation*}
    -r_\lambda ^{a - 1}\sum\limits_{i=1}^N\sum\limits_{j=1}^K \beta_{i,j}(w_\lambda)\nabla_wf_w(x_i)[j]|_{w=\frac{w_\lambda}{r_\lambda}}+2\lambda w_\lambda = 0.
\end{equation*}
Dividing the equality by $2\lambda r_\lambda$ and noting that $w_\lambda = r_\lambda \hat w + o(r_\lambda)$, we have:
\begin{equation*}
    -\frac {r_\lambda^{a - 2}}{2\lambda}\sum\limits_{i=1}^N\sum\limits_{j=1}^K\beta_{i,j}(w_\lambda)\nabla_wf_{w}(x_i)[j]|_{w=\frac{w_\lambda}{r_\lambda}} + \hat w = o(1).
\end{equation*}
Note that $f$ is continuously-differentiable, so we know $\lim\limits_{\lambda\rightarrow 0^+}\nabla_wf_{w}(x_i)[j]|_{w=\frac{w_\lambda}{r_\lambda}}=\nabla_wf_{w}(x_i)[j]|_{w=\hat w}$, which are linearly independent for $1\leq i\leq N,1\leq j\leq K$. Therefore, $\max_{1\leq i \leq N,1\leq j\leq K}\left|-\frac{r_\lambda^{a - 2}}{2\lambda}\beta_{ij}(w_\lambda)\right|$ is bounded uniformly for $\lambda$ sufficiently close to $0^+$. Consequently,
\begin{equation*}
    -\frac {r_\lambda^{a - 2}}{2\lambda}\sum\limits_{i=1}^N\sum\limits_{j=1}^K\beta_{i,j}(w_\lambda)\nabla_wf_{w}(x_i)[j]|_{w=\hat w} + \hat w = o(1).
\end{equation*}
Therefore, $\forall 1\leq i\leq N,1\leq j\leq K$ we have $\lim\limits_{\lambda\rightarrow 0^+}\frac{r_\lambda^{a - 2}}{2\lambda}\beta_{i,j}(w_\lambda)=\alpha_{i,j}$, where $\sum\limits_{i=1}^N\sum\limits_{j=1}^K\alpha_{i,j}\nabla_wf_{w}(x_i)[j]|_{w=\hat w}=\hat w$. 

Note that $\forall 1\leq i\leq N,\forall w\in\bb R^d,\sum_{j=1}^K\beta_{i,j}(w)=0$, and $\beta_{i,y_i}>0>\beta_{i,j}$ for $j\neq y_i$. Therefore, $\forall 1\leq i\leq N,\sum_{j=1}^K\alpha_{i,j}=0$ and $\alpha_{i,y_i}\geq 0\geq \alpha_{i,j}$ for $j\neq y_i$. Therefore, $\sum_{i=1}^N\alpha_{i,y_i}>0$, because otherwise we would get $\alpha_{i,j}=0$ for all $1\leq i\leq N,1\leq j\leq K$, a contradiction with $\hat w\neq 0$.

Now we have $\forall 1\leq i\leq N$,
\begin{equation}
\label{eq:beta_ratio}
    \lim\limits_{\lambda \rightarrow 0^+}\frac{\beta_{i,y_i}(w_\lambda)}{\sum_{j=1}^N\beta_{j,y_j}(w_\lambda)}=\frac{\alpha_{i,y_i}}{\sum_{j=1}^N\alpha_{j,y_j}}.
\end{equation}
Finally, note that
\begin{align*}
\lim_{\lambda\rightarrow 0^+}\frac{\ell(f_{w_\lambda}(x_i),y_i)}{\beta_{i,y_i}(w_\lambda)}=&\lim_{\lambda\rightarrow 0^+}\ell(f_{w_\lambda}(x_i),y_i)\cdot \frac{\sum_{1\leq k\leq K}\exp(f_{w_\lambda}(x_i)[k])}{\sum_{1\leq k\leq K,k\neq y_i}\exp(f_{w_\lambda}(x_i)[k])}\\
=&\lim_{\lambda\rightarrow 0^+}\ell(f_{w_\lambda}(x_i),y_i)\cdot\frac{\exp(f_{w_\lambda}(x_i)[y_i])}{\sum_{1\leq k\leq K,k\neq y_i}\exp(f_{w_\lambda}(x_i)[k])}\cdot\frac{\sum\limits_{1\leq k\leq K}\exp(f_{w_\lambda}(x_i)[k])}{\exp(f_{w_\lambda}(x_i)[y_i])}\\
=&\lim_{\lambda\rightarrow 0^+}\ell(f_{w_\lambda}(x_i),y_i)\cdot\frac{\exp(f_{w_\lambda}(x_i)[y_i])}{\sum_{1\leq k\leq K,k\neq y_i}\exp(f_{w_\lambda}(x_i)[k])}\\
=&\lim_{\lambda\rightarrow 0^+}\ln\left(1+\frac{\sum_{1\leq k\leq K,k\neq y_i}\exp(f_{w_\lambda}(x_i)[k])}{\exp(f_{w_\lambda}(x_i)[y_i])}\right)\cdot \frac{\exp(f_{w_\lambda}(x_i)[y_i])}{\sum_{1\leq k\leq K,k\neq y_i}\exp(f_{w_\lambda}(x_i)[k])}\\
=&\lim\limits_{\lambda\rightarrow 0^+}\frac{\sum_{1\leq k\leq K,k\neq y_i}\exp(f_{w_\lambda}(x_i)[k])}{\exp(f_{w_\lambda}(x_i)[y_i])}\cdot \frac{\exp(f_{w_\lambda}(x_i)[y_i])}{\sum_{1\leq k\leq K,k\neq y_i}\exp(f_{w_\lambda}(x_i)[k])}\\
=&1,
\end{align*}
which further implies $\lim\limits_{\lambda\rightarrow 0^+}\frac{\sum_{j=1}^N\ell(f_{w_\lambda}(x_j),y_j)}{\sum_{j=1}^N\beta_{j,y_j}(w_\lambda)}=1$. Combining with (\ref{eq:beta_ratio}), we get
the desired equality.
\end{proof}

==> strong_lm_3.tex <==
\section{Original proof of Lemma 3}
\begin{lemma}
\label{lm:sgd_max_margin}
% Suppose we have $N$ training examples, $(x_1,y_1),(x_2,y_2),\cdots,(x_N,y_N)\in\bb R^d\times\{\pm 1\}$. Assume $x_1,x_2,\cdots,x_N$ are linearly independent. Suppose we train a linear model $f_w(x)=w^\top x$ using Stochastic Gradient Descent on the objective $\sum_{i=1}^N\ell(y_if_w(x_i))$ using constant learning rate $\eta$, where the loss function $\ell(\cdot)$ is the logistic loss $\ell(z)=\ln(1+\exp(-z))$, and get iterate $w_t$ after iteration $t$. 
In the setting of Lemma \ref{lm:sgdratio}, assume each epoch consists of $K$ iterations each corresponding to a minibatch of size $B=N/K$. %, and in each epoch every training example is selected in exactly one minibatch.  
% We define $\gamma(w)$ to be the margin of $w$ on the training set: $\gamma(w)=\min_{1\leq i\leq N}y_if_w(x_i)$, and $\hat w$ to be the max-margin solution: $\hat w = \argmin\{\|w\|_2:\gamma(w)\geq 1\}$. 
Define $X=[y_1x_1,y_2x_2,\cdots,y_Nx_N]\in\bb R^{d\times N}$. Then, there exists a unique $\bm \alpha = (\alpha_1,\alpha_2,\cdots,\alpha_N)^\top \in\bb R^N$ such that $X^\top X\bm\alpha = (1,1,\cdots,1)^\top$. Moreover, if every $\alpha_i$ is positive and
\begin{equation}
\label{eq:small_rate}
    \eta < \min\left\{\frac 1{2K\beta\sigma_{\max}^2(X)}, \frac {\gamma^*}{2\beta\sigma^3_{\max}(X)(K+\sigma_{\max}(X)/\gamma^*)}\right\},
\end{equation}
where $\gamma^*=\left(\sum_{i=1}^N\alpha_i\right)^{-1/2}$ is the maximum normalized margin and $\beta = \frac 14$ is the smoothness coefficient of $\ell(\cdot)$, then for any initialization $w_0\in\bb R^d$, there exists $\tilde w\in\bb R^d$ satisfying $\forall i,\exp(-y_i\tilde w^\top x_i)=\frac{\alpha_i}\eta$ and 
\begin{equation*}
    \lim\limits_{t\rightarrow +\infty}\left\|w_t-\ln\left(\frac tK\right)\hat w-\tilde w\right\|_2=0,
\end{equation*}
where $\hat w = X\bm\alpha$.

% Assume the examples are linearly separable with max-margin solution $\hat w\neq \mathbf 0$ and corresponding dual solutions $\alpha_1,\alpha_2,\cdots,\alpha_m\in\bb R_{> 0}$ satisfying $\sum_{i=1}^m\alpha_iy_ix_i=\hat w$. Note that here we assume $\alpha_i>0$ for every $i$, which implies every example $(x_i,y_i)$ is a ``support vector'', i.e., $y_i\hat w^\top x_i=1$. Let $\ell(w;x,y)=\ell(yw^\top x)=\ln(1+\exp(-yw^\top x))$ be the Logistic loss. Suppose $w_0\in\bb R^d$ is any initialized weight. For any $t\in\bb N^*$, at time step $t$, we update $w_{t-1}$ to $w_t$ using Stochastic Gradient Descent with batch $B(t)\subseteq \{1,2,\cdots,m\}$:
% \begin{equation}
% \label{eq:sgd_update}
%     w_t=w_{t-1} - \eta\sum\limits_{i\in B(t)}\nabla_w\ell(w_{t-1};x_i,y_i).
% \end{equation}
% Here $\eta\in\bb R_{>0}$ is the learning rate. Suppose each epoch has $K$ iterations, and for every $p\in\bb N^*$, $B(pK-K+1),B(pK-K+2),\cdots,B(pK)$ form a partition of $\{1,2,\cdots,m\}$. Assume the learning rate satisfies
% \begin{equation*}
%     \eta < \min\{\frac 1{2K\beta\sigma_{\max}^2}, \frac r{2\beta\sigma^3_{\max}(K+r ^{-1}\sigma_{\max})}\},
% \end{equation*}
% where $r = \frac 1{\|\hat w\|}$, $\beta$ is the smoothness coefficient of the Logistic loss and $\sigma_{\max}$ is the maximum singular value of the matrix $[x_1,x_2,\cdots,x_m]\in\bb R^{d\times m}$.

% Then, there exist $\tilde w\in\bb R^d$ satisfying $\forall i,\exp(-y_i\tilde w^\top x_i)=\frac{\alpha_i}{\eta}$ and
% \begin{equation*}
%     \lim\limits_{t\rightarrow +\infty}\left\|w_t-\ln\left(\frac tK\right)\hat w-\tilde w\right\|=0
% \end{equation*}
\end{lemma}

\begin{proof}
Since $x_1,x_2,\cdots,x_N$ are linearly independent, $X$ has full column rank and $X^\top X$ is invertible. This proves the existence and uniqueness of $\bm\alpha$. Let's now focus on the case where every $\alpha_i$ is positive and the learning rate satisfies (\ref{eq:small_rate}).

Consider the following hard-margin SVM problem:
\begin{align*}
    \text{Minimize }&\frac 12\|w\|_2^2,\\
    \text{s.t. }&\forall 1\leq i\leq N, y_iw^\top x_i\geq 1.
\end{align*}
By definition, $X^\top \hat w=X^\top X\bm\alpha = (1,1,\cdots,1)^\top$. Therefore, $\hat w$ is a feasible solution to the above optimization problem with objective value $\frac 12\|\hat w\|_2^2=\frac 12\hat w^\top \hat w=\frac 12\bm\alpha^\top X^\top X\bm\alpha=\frac 12\bm\alpha^\top (1,1,\cdots,1)^\top=\frac 12\sum_{i=1}^N\alpha_i$. Moreover, $\bm\alpha$ is a feasible solution to the dual:
\begin{align*}
    \text{Maximize }&\sum_{i=1}^N\alpha_i-\frac 12\sum_{i=1}^N\sum_{j=1}^N\alpha_i\alpha_jy_iy_jx_i^\top x_j,\\
    \text{s.t. }&\forall 1\leq i\leq N,\alpha_i\geq 0,
\end{align*}
with objective value $\sum_{i=1}^N\alpha_i-\frac 12\bm\alpha^\top X^\top X\bm\alpha=\sum_{i=1}^N\alpha_i-\frac 12\bm\alpha^\top (1,1,\cdots,1)^\top=\frac 12\sum_{i=1}^N\alpha_i$. Therefore, $\hat w$ is the global optimum of the primal and $\bm\alpha$ is the global optimum of the dual. By complementary slackness, every $\alpha_i$ being positive means every training example being a support vector. Moreover, $\gamma^* = \left(\sum_{i=1}^N\alpha_i\right)^{-1/2} = \|\hat w\|_2^{-1}$ equals to the maximum normalized margin $\max_{\|w\|_2 = 1}\min_{1\leq i\leq N}y_iw^\top x_i$.

Now let's show that we can assume $w_0\in\Span(x_1,x_2,\cdots,x_N)$ without loss of generality. Otherwise, say $w_0=w^\perp+w_0'$ where $w_0'\in\Span(x_1,x_2,\cdots,x_N)$ and $w^\perp \perp \Span(x_1,x_2,\cdots,x_N)$. Then, the SGD update rule ensures that for every $t$, $w_t=w^\perp + w_t'$ where $w_t'\in\Span(x_1,x_2,\cdots,x_N)$. Moreover, the sequence $w_t'$ also follows the SGD update rule. If we could prove the lemma for $w_0'$, i.e., there exists $\tilde w'\in\bb R^d$ satisfying $\forall i,\exp(-y_i(\tilde w')^\top x_i)=\frac{\alpha_i}{\eta}$ and $\lim\limits_{t\rightarrow +\infty}\|w_t'-\ln(\frac tK)\hat w - \tilde w'\|_2=0$, then taking $\tilde w=\tilde w'+w^\perp$ yields a proof for $w_0$.

Now we assume $w_0\in\Span(x_1,x_2,\cdots,x_N)$ without loss of generality. Note that we have assumed $x_1,x_2,\cdots,x_N$ to be linearly independent, so there exists a unique $\tilde w\in\Span(x_1,x_2,\cdots,x_N)$ satisfying $\forall i,\exp(-y_i\tilde w^\top x_i)=\frac{\alpha_i}{\eta}$. Now we only need to show that $\lim\limits_{t\rightarrow +\infty}\|w_t-\ln(\frac tK)\hat w-\tilde w\|_2=0$.

Note that we can also assume $y_i=1$ for $1\leq i\leq N$ without loss of generality by replacing $y_ix_i$ by a new $x_i$. Define $B(u)$ to be the set of indices of training examples selected in the minibatch corresponding to the $u$th iteration. By Lemma 5 in \cite{nacson2018stochastic}, we know that $\ln(\frac tK)\hat w=K\sum\limits_{u=1}^{t-1}\frac 1u\sum\limits_{n\in B(u)}\alpha_nx_n-\gamma \hat w+o(1)$ as $t\rightarrow +\infty$, where $\gamma$ is the Euler-Mascheroni constant. %where $\|m_4(t)\|=o(t^{-0.5})$. 
Therefore, we only need to show that $\lim\limits_{t\rightarrow +\infty}\|r(t)\|_2=0$, where 
\begin{equation*}
    r(t)=w_t-K\sum\limits_{u=1}^{t-1}\frac 1u\sum\limits_{n\in B(u)}\alpha_nx_n+\gamma\hat w-\tilde w.
\end{equation*}

In Section B.1, \citet{nacson2018stochastic} showed that $\sum_{t=0}^{+\infty}\|r(t+1)-r(t)\|_2^2<\infty$. Lemma 6 in \cite{nacson2018stochastic} showed that there exist $c_1,\delta>0$ such that for all $t\in\bb N^*$, it holds that
\begin{equation*}
    (r(t+1)-r(t))^\top r(t)\leq c_1t^{-1-\delta}.
\end{equation*}
Therefore, $\forall \varepsilon > 0$, we can find $t_1\in\bb N^*$ such that $\forall t',t''\in\bb N^*\text{ with }t''>t'\geq t_1$,
\begin{align}
&\|r(t'')\|_2^2-\|r(t')\|_2^2\nonumber \\
   =&\sum\limits_{t=t'}^{t''-1}(\|r(t+1)\|_2^2-\|r(t)\|_2^2)\nonumber \\
  =&\sum\limits_{t=t'}^{t''-1}(\|r(t+1)-r(t)\|_2^2+2(r(t+1)-r(t))^\top r(t))\nonumber \\
  \leq &\sum\limits_{t=t'}^{t''-1}\|r(t+1)-r(t)\|_2^2+2c_1\sum\limits_{t=t'}^{t''-1}t^{-1-\delta}\nonumber \\
  \leq & \varepsilon.  \label{eq:partialsum}
\end{align}

Now we show that there exist $c_2>0$ and $t_2\in\bb N^*$ such that for all $t\geq t_2$ with $\|r(t)\|_2\geq \varepsilon$, there exists $t'\in\bb N^*$ with $t\leq t'<t+2K$ satisfying $(r(t'+1)-r(t'))^\top r(t')\leq -c_2t^{-1}$. Note that $x_1,\cdots,x_N$ are linearly independent, so $X^\top$ has a minimum positive singular value $\sigma_{\min}:=\min_{r\in\Span\{x_1,\cdots,x_N\}:\|r\|_2=1}\|X^\top r\|_2>0$ and thus
$\|X^\top r(t)\|_2\geq \sigma_{\min}\|r(t)\|_2\geq \sigma_{\min}\varepsilon$.
Therefore, there exists $i_1$ such that 
$|x_{i_1}^\top r(t)|\geq \varepsilon_1:=\frac{\sigma_{\min} \varepsilon}{\sqrt N}$.
By picking $t_2$ sufficiently large, we can ensure that for every $t\geq t_2$, it holds that $\|r(t+1)-r(t)\|_2\leq \frac{\varepsilon_1}{4K(\max_{1\leq i\leq N}\|x_i\|_2)}$. Then, $\forall t'\in\bb N^*$ with $t\leq t'<t+2K$, we have $|x_{i_1}^\top r(t')|\geq |x_{i_1}^\top r(t)|-|x_{i_1}^\top (r(t)-r(t'))|\geq \varepsilon_1-\|x_{i_1}\|_2\|r(t)-r(t')\|_2\geq \frac{\varepsilon_1} 2$. Pick $t'$ so that $i_1\in B(t')$. In Section B.2, \citet{nacson2018stochastic} showed that
\begin{equation}
\label{eq:decomposition}
    (r(t'+1)-r(t'))^\top r(t')\leq \sum\limits_{i\in B(t')}\alpha_i\frac K{t'}(\gamma_i(t')\exp(\tilde m_i(t')-x_i^\top r(t'))-1)x_i^\top r(t')
\end{equation}
as long as we pick $t_2$ sufficiently large, where $\tilde m_i(t)\rightarrow 0$ and $\gamma_i(t)\rightarrow 1$ as $t\rightarrow +\infty$. In Section B.2, \citet{nacson2018stochastic} also showed that there exist $c',\delta'\in\bb R_{>0}$ independent of $t,t'$ such that $\forall 1\leq i\leq N$
\begin{equation}
\label{eq:positive}
    \alpha_i\frac K{t'}(\gamma_i(t')\exp(\tilde m_i(t')-x_i^\top r(t'))-1)x_i^\top r(t')\leq c'(t')^{-1-\delta'}\leq c't^{-1-\delta'}.
\end{equation}
Now we show that there exists $c_2'\in\bb R_{>0}$ independent of $t,t'$ such that 
\begin{equation}
\label{eq:negative}
    \alpha_{i_1}\frac K{t'}(\gamma_{i_1}(t')\exp(\tilde m_{i_1}(t')-x_{i_1}^\top r(t'))-1)x_{i_1}^\top r(t')\leq -c_2'(t')^{-1}\leq -c_2'(t+2K)^{-1}.
\end{equation}
When $x_{i_1}^\top r(t')\geq \frac{\varepsilon_1}{2}$, as long as we pick $t_2$ sufficiently large, we can make sure that $\gamma_{i_1}(t')\exp(\tilde m_{i_1}(t')-x_{i_1}^\top r(t'))-1\leq \exp(-\frac{\varepsilon_1}{4})-1$, so the left hand side of (\ref{eq:negative}) is upper bounded by $-\alpha_{i_1}\frac K{t'}\frac{\varepsilon_1}{2}(1-\exp(-\frac{\varepsilon_1}{4}))$. Similarly, when $x_{i_1}^\top r(t')\leq -\frac{\varepsilon_1}{2}$, as long as we pick $t_0$ sufficiently large, we can make sure that $\gamma_{i_1}(t')\exp(\tilde m_{i_1}(t')-x_{i_1}^\top r(t'))-1\geq \exp(\frac{\varepsilon_1}{4})-1$, so the left hand side of (\ref{eq:negative}) is again upper bounded by $-\alpha_{i_1}\frac K{t'}\frac{\varepsilon_1}{2}(\exp(\frac{\varepsilon_1}{4})-1)\leq -\alpha_{i_1}\frac K{t'}\frac{\varepsilon_1}{2}(1-\exp(-\frac{\varepsilon_1}{4}))$. Therefore, we can choose $c_2'=(\min_{1\leq i\leq N}\alpha_{i})K\varepsilon_1(1-\exp(\varepsilon_1/4))/2$.

Combining (\ref{eq:positive}) and (\ref{eq:negative}) with (\ref{eq:decomposition}), we know
\begin{equation*}
    (r(t'+1)-r(t'))^\top r(t')\leq |B(t')|c't^{-1-\delta'}-c_2'(t+2K)^{-1}\leq c'Nt^{-1-\delta'}-c_2'(t+2K)^{-1}.
\end{equation*}
Now as long as we pick $t_2$ sufficiently large, we know there exists $c_2>0$ independent of $t,t'$ such that $(r(t'+1)-r(t'))^\top r(t')\leq -c_2t^{-1}$.

Suppose $\|r(t)\|_2\geq\varepsilon$ for all $t\geq \max\{t_1,t_2\}$. Then 
\begin{align*}
&\sum\limits_{t\geq \max\{t_1,t_2\}}(\|r(t+1)\|_2^2-\|r(t)\|_2^2)\\
=&\sum\limits_{t\geq \max\{t_1,t_2\}}\|r(t+1)-r(t)\|_2^2+2\sum\limits_{t\geq \max\{t_1,t_2\}}(r(t+1)-r(t))^\top r(t)\\
\leq &\varepsilon+2c_1\sum\limits_{t\geq \max\{t_1,t_2\}}t^{-1-\delta}-2c_2\sum\limits_{t\geq \max\{t_1,t_2\}\atop t\text{ is a multiple of }2K}t^{-1}\\
=&-\infty,
\end{align*}
a contradiction. Therefore, there exists $t_3\geq \max\{t_1,t_2\}$ with $\|r(t_3)\|_2\leq \varepsilon$. Now for any $t\geq t_3$, we have $\|r(t)\|_2^2\leq \varepsilon^2+\varepsilon$ according to (\ref{eq:partialsum}). By the arbitrariness of $\varepsilon>0$, we have proved $\lim\limits_{t\rightarrow +\infty}\|r(t)\|_2=0$.
\end{proof}


==> tables/tables.tex <==
\begin{table*}[htbp]
\begin{center}
\caption{Minimum validation error throughout training (in percentage).}
\label{tab:cifar-val}
\begin{tabular}{c|ccc|ccc}
\toprule
& \multicolumn{3}{c|}{CIFAR-10} & \multicolumn{3}{c}{CIFAR-100} \\
\multirow{2}{*}{Method} & \multicolumn{3}{c|}{$\%$ of Mislabeled Examples} & \multicolumn{3}{c}{$\%$ of Mislabeled Examples} 
\\
                                             & 0                              & 20                              & 40                & 0 & 20 & 40             \\\midrule
 \textsc{Oracle}                                      & - & $4.25 \pm 0.05$  & $5.06 \pm 0.05$  & - & $20.42 \pm 0.20$  & $23.64 \pm 0.27$  \\\midrule
\textsc{ERM}                                           & $3.73 \pm 0.13$ & $11.53 \pm 0.06$ & $15.57 \pm 0.45$ &  $18.41 \pm 0.17$ & $30.38 \pm 0.14$ & $44.35 \pm 0.53$ \\
\textsc{ODD}                              & $3.80 \pm 0.10$ & $\textbf{5.33} \pm 0.04$  & $\textbf{7.16} \pm 0.20$ & $\textbf{18.19} \pm 0.10$ & $\textbf{22.79} \pm 0.10$  & $\textbf{27.61} \pm 0.38$    \\
\textit{mixup}                                                &           $\textbf{3.04} \pm 0.05$     & $6.09 \pm 0.27$ & $9.26 \pm 0.14$  & $18.61 \pm 0.33$ & $28.78 \pm 0.27$ & $40.58 \pm 0.35$  \\
\textsc{GCE}     &  -  & $10.13 \pm 0.20$  & $12.87 \pm 0.22$  & - & $33.19 \pm 0.42$ & $38.23 \pm 0.24$ \\\midrule
\textsc{Ren}$^\star$   &    -    &    -     & $13.08 \pm 0.19$ & - & - & $38.66 \pm 2.06$  \\\midrule
\textsc{MentorNet} & - & 9 & 23     & - & 28 & 44                   \\
\textsc{MentorNet}$^\star$ &   -      & 8    & 11  & - & 27 & 32 \\\bottomrule                          
\end{tabular}
\end{center}
\end{table*}
